Hyperion: Unveiling DApp Inconsistencies using LLM and Dataflow-Guided Symbolic Execution

The rapid advancement of blockchain platforms has significantly accelerated the growth of decentralized applications (DApps). Similar to traditional applications, DApps integrate front-end descriptions that showcase their features to attract users, and back-end smart contracts for executing their business logic. However, inconsistencies between the features promoted in front-end descriptions and those actually implemented in the contract can confuse users and undermine DApps's trustworthiness. In this paper, we first conducted an empirical study to identify seven types of inconsistencies, each exemplified by a real-world DApp. Furthermore, we introduce HYPERION, an approach designed to automatically identify inconsistencies between front-end descriptions and back-end code implementation in DApps. This method leverages a fine-tuned large language model LLaMA2 to analyze DApp descriptions and employs dataflow-guided symbolic execution for contract bytecode analysis. Finally, HYPERION reports the inconsistency based on predefined detection patterns. The experiment on our ground truth dataset consisting of 54 DApps shows that HYPERION reaches 84.06% overall recall and 92.06% overall precision in reporting DApp inconsistencies. We also implement HYPERION to analyze 835 real-world DApps. The experimental results show that HYPERION discovers 459 real-world DApps containing at least one inconsistency.

==> icse2025-p517/01_intro.tex <==
\section{Introduction}
%Over recent years, diverse decentralized applications (DApps)~\cite{wu2019empirical, werner2022sok, nftdefects} built on blockchains~\cite{zheng2020overview} have experienced a significant surge in popularity and market capitalization~\cite{etherscan}.
%Notably, in 2023, the total value locked in the DApps reached \$83.3 billion~\cite{dappcap}.
In recent years, the blockchain industry has witnessed a remarkable proliferation of various decentralized applications (DApps), which have gained substantial popularity and market capitalization~\cite{wu2019empirical, werner2022sok, nftdefects}. 
Similar to traditional applications like web or Android apps, a DApp utilizes a user interface (UI) as its front-end to present feature descriptions and employs smart contracts for back-end logic execution.


However, inconsistency between the front-end descriptions and the actual implementation of their back-end contract code of DApps may have detrimental consequences~\cite{duan2022towards}.
% 举一个不一致的问题，然后说明当前工作的特别之处
For example, a DApp might advertise a 3\% investment return in its description, but the actual return could be changed (lower than 3\%) after investment.
% However, the exact return that users can obtain depends on the contract balance and some other undetermined factors that are unknown at the time when the user invests in the DApp.
%Additionally, hidden fees in the contract, not mentioned in the DApp’s description, can also unexpectedly reduce user returns.
Similarly, in the case of some NFT DApps, the front-end description may claim that NFTs can ``live forever'', while in reality, the metadata of these NFTs is stored on centralized servers, which are susceptible to shutdown. These inconsistencies can pose threats to users' interests and undermine the trustworthiness of DApps.  

Many research efforts have been made to detect vulnerabilities in smart contracts to ensure their safety~\cite{luu2016making,nftdefects,tsankov2018securify,choi2021smartian,jiang2018contractfuzzer}.
However, they usually overlook the importance of inconsistencies between the front-end descriptions and back-end implementations in DApps. For instance, consider a scenario where a DApp offers users a 2\% interest rate and does not mention fees; traditional vulnerability detection tools may not flag this as an issue. However, when the promised rates in the DApp's description do not align with this or fees are charged secretly, it can indicate dishonest behavior of the DApps' owners and pose potential risks to DApp users.

% These inconsistencies between DApp descriptions and smart contract implementation may confuse users, leading to financial losses and eroding trust in DApps.
% As misleading information shown in the DApp
% descriptions may influence users' investment decisions or make them lose the money they invest and ruin the trustworthiness of DApps.
% % 怎么突出一个对比
%Previous works have studied whether the transaction generated from DApp's UI is consistent with contract transaction log, and check whether DApp contracts conform to the safety specification inferred from UI widgets.
% Previous research has explored the use of DApp front-end buttons to trigger transactions, thereby identifying inconsistencies~\cite{zhou2023dapphunter}, and applying safety checking rules to UI widgets for contract analysis in specific DApp category~\cite{duan2022towards}.
% However, the front-end information they focus on may miss some critical information related to the user assets shown in the DApp descriptions (see Section~\ref{bg:sc}). 
The detection of DApp inconsistencies presents unique challenges.
First, there is no systematic work aimed at uncovering the various types of inconsistencies within the DApp ecosystem. This absence makes it not easy to design rules to detect inconsistencies. Second, the diverse and intricate structures of DApp front-end descriptions present considerable difficulties when attempting to extract information related to user assets.
Third, it is challenging to recover the semantics from the contract code effectively. Many malicious DApp developers may not disclose their source code on Ethereum~\cite{liao2022smartdagger}. Consequently, detecting inconsistencies from the bytecode level is crucial, but also increases the difficulty.
% Although there are some binary analysis works that recover program behaviors based on APIs (e.g., \textit{getInstalledPackages()} in Android Apps)~\cite{yu2018ppchecker,DiffDroid,ocariza2017detecting,datausage}, these types of API are absent in smart contract programming languages.


To address these challenges, we first conducted an empirical study employing an open card sorting approach~\cite{spencer2009card} to find DApp inconsistencies. This involved analysis of both the front-end descriptions and the smart contracts of a dataset comprising 321 DApps (see Section~\ref{sec:define}). Based on this approach, we define seven types of DApp inconsistencies that encompass both DeFi and NFT DApps, namely \textit{Unguaranteed Reward}, \textit{Hidden Fee}, \textit{Adjustable Liquidity}, \textit{Unconstrained Token Supply}, \textit{Unclaimed Fund Flow}, \textit{Changeable DApp Status}, and \textit{Volatile NFT Accessibility}.
% Furthermore, although there are several works on the inconsistency detection of DApps, they still have limitations.
% For the DApp front-end analysis, they focus on some widgets or buttons that can trigger transactions on the DApp UI~\cite{duan2022towards,zhou2023dapphunter}, which may miss some critical information related to the user assets shown in the DApp descriptions (see Section~\ref{bg:sc}).
% Some works do not analyze contract code, but rely on transaction information~\cite{zhou2023dapphunter}, which may miss some contract behaviors.
% Furthermore, there is no systematic work to unveil what inconsistencies exist in the DApp ecosystem and an understanding of their manifestation.

To automatically detect these inconsistencies, we propose a tool named \textsc{Hyperion}, which contains a description analyzer \textsc{HyperText} and a contract analyzer \textsc{HyperCode}.
\textsc{HyperText} leverages LLaMA2~\cite{touvron2023llama}, a widely-recognized, public-available large language model~\cite{chen2023chatgpt} (LLM), to scrutinize the diverse natural language descriptions found on DApp websites. 
To optimize LLaMA2 for the specific domain task, i.e., extract critical attributes from the DApp front-end descriptions, we first design a prompt template based on the chain of thought~\cite{wei2023chainofthought} (CoT) prompting technique, tailored to our identified inconsistency types. Then, we manually label a dataset containing 63 DApp inconsistencies to fine-tune LLaMA2 (see Section~\ref{sec:fine-tune}), thereby enhancing its performance for our downstream task and obtaining our model \textsc{HyperText}. Finally, we employ the Natural Language Tool Kit~\cite{nltk} (NLTK) to extract inconsistency-related attributes from \textsc{HyperText}'s output (see Section~\ref{sec:nltk}).


% The output of our \textsc{Hyperion} can help DApp developers find issues in the alignment of the DApp website design and contract development, assist DApp users in assessing the trustworthiness of a DApp, and enable DApp marketplaces to identify risky DApps.

% The design and development of \textsc{Hyperion} presents unique challenges.
% First, the diverse and complex structures of DApp websites make extracting user asset-related information difficult.
% Second, \textsc{Hyperion} should be able to analyze contract behavior from bytecode, as malicious DApps may not reveal their contract source code, and more than 99\% smart contracts do not disclose their source code on Ethereum~\cite{liao2022smartdagger}. 
% Therefore, how to effectively recover the contract semantics from its bytecode is an essential problem. 
% Although there are some binary analysis works that recover program behaviors based on APIs (e.g., \textit{getInstalledPackages()} in Android Apps)~\cite{yu2018ppchecker,DiffDroid,ocariza2017detecting,datausage}, these types of API are absent in smart contract programming languages.


% To address these challenging issues, \textsc{Hyperion} uses LLaMA2~\cite{touvron2023llama}, a popular public-available large language model (LLM), effective in processing and understanding natural language. This enables us to analyze varied textual information on DApp websites.

For the analysis of DApp contract bytecode, \textsc{HyperCode} employs an approach that utilizes dataflow analysis to guide symbolic execution on the contract intermediate representation (IR), so as to obtain relevant program states and recover contract semantics (see Section~\ref{sec:sca}).
Specifically, \textsc{HyperCode} first decompiles the contract bytecode and performs dataflow analysis to recover low-level semantics such as contract call and state variable storage access operations.
Then, it performs a graph analysis based on the recovered semantics to obtain the contract's fund transfer and state variable dependency relationship.
To obtain contract semantics, \textsc{HyperCode} proposes a symbolic execution framework based on contract IR. This framework utilizes dataflow and graph analysis to optimize search paths and direct symbolic execution to check relevant program states, merging the strengths of both methods.
% For DApp contract bytecode analysis, we employ an approach that utilizes dataflow analysis to guide symbolic execution on the contract intermediate representation (IR) (see Section~\ref{sec:sca}). This approach optimizes the search for relevant program points using data flow analysis to direct symbolic execution to check program states, effectively merging the strengths of both methods.
Furthermore, we propose algorithms that compare the information extracted from DApp descriptions and contract semantics based on this framework to detect the seven defined inconsistencies, unveiling whether one DApp's \textit{saying} is consistent with its \textit{doing}.

To evaluate the performance of \textsc{Hyperion}, we first collect two datasets; one serves as the ground truth dataset, containing  \DAppGT~labeled DApps used to define DApp inconsistencies and evaluate the effectiveness of the \textsc{Hyperion}. The other dataset is used to evaluate the performance of \textsc{Hyperion} on analyzing real-world wild DApps, which contains \WildDApp~real-world DApps collected from DappBay~\cite{DappBay} and DappRadar~\cite{DappRadar}.
\textsc{Hyperion} reaches an overall recall of \OverallRecall~and an overall precision of 92.06\% in the first ground truth dataset. Furthermore, \textsc{Hyperion} identifies \WildHasOne~out of \WildDApp~DApps with at least one inconsistency that we define in the second large-scale dataset, with an overall precision of \OverallPrecision~in our sampled dataset.
Among the true positives (268 DApps) in the sampled dataset, we find that 67 (25\%) DApps' websites become inaccessible within only 3 months.

% The experiment on \WildDApp~real-world DApps collected from DAppBay and DAppRadar shows that \textsc{Hyperion} identifies \WildHasOne~DApps with at least one inconsistency that we define, with an overall precision of \OverallPrecision.
% \textsc{Hyperion} output helps DApp developers align website design and contract development, assists users in assessing DApp trustworthiness, and enables marketplaces to identify risky DApps, providing a new insight into the DApp ecosystem.


In summary, the contributions of our paper are as follows:
\begin{itemize}
\item We define seven common inconsistency types between DApp front-end description and back-end smart contract implementation. To enhance comprehension, we illustrate each inconsistency with a real-world DApp example and its consequences.
\item We design and develop \textsc{Hyperion}, a tool that leverages LLM and dataflow-guided symbolic execution to automatically detect defined inconsistencies. %The experiment results on \WildDApp~real-world DApps demonstrate that \textsc{Hyperion} reaches a precision of \OverallPrecision~in finding the 7 types of DApp inconsistencies.%We have conducted extensive experiments to construct a fine-tuned and effective LLM so as to extract information from diverse DApp descriptions.
%The contract analysis approach proposes an extensible framework that combines dataflow analysis with symbolic execution on contract IR.
% \item The experiment results on \WildDApp~real-world DApps demonstrate that \textsc{Hyperion} reaches a precision of \OverallPrecision~in finding the 7 types of DApp inconsistencies, highlighting its effect in practical scenarios.
\item We find \WildHasOne~out of \WildDApp~DApps in our dataset contain at least one inconsistency, which demonstrates the prevalence of the defined inconsistencies in the DApp ecosystem.

\item To promote further research and transparency, we have released the source code of \textsc{Hyperion} (both fine-tuned \textsc{HyperText} and \textsc{HyperCode}) as well as the DApp dataset resources and experimental results in the repository {\href{https://github.com/shuo-young/Hyperion}{https://github.com/shuo-young/Hyperion}}.

\end{itemize}

% 人工检查很费时间
% Therefore, given an app and its privacy policy, user may wonder whether they can trust the privacy policy or not. Although manually dissecting apps and scrutinizing the privacy policies could answer this question, it is time-consuming.


% Decentralized Applications (DApps) represent a transformative approach to software, offering decentralized control, robustness against censorship, and seamless integration with blockchain technologies. As with all applications, the user interface and, more importantly, the front-end description, play pivotal roles in user adoption.


% However, there is no general work that identifies what kind of inconsistencies exist in the DApp ecosystem, and how to automatically detecting those inconsistencies without more manual effort for design rules for a specific DApp.
% Some work checks whether a smart contract is implemented correctly according to designed rules of a specific DApp type, e.g., auction, identified from front-end widgets.
% either do not analyze contract bytecode, or just analyze part of the description. In addition, they do not pay attention to the specific fund-related operations which are mostly related to the DApp security.

==> icse2025-p517/02_background.tex <==
\vspace{-0.2cm}
\section{Background}
\subsection{DApp and Smart Contract}
Decentralized applications (DApps) typically leverage smart contract technology to achieve autonomous and transparent operations~\cite{zhou2023dapphunter,zheng2020overview}.
%DeFi~\cite{werner2022sok} and NFT~\cite{nftdefects} are the two main DApp types that prevail in the DApp ecosystem.
A DApp usually uses a user interface (UI) that showcases its functionalities to attract users. Some financial-related features, such as return on investment (ROI), token supply, and liquidity, are central to user interest and are implemented within the smart contract. Smart contracts are commonly written in high-level programming languages, e.g., Solidity~\cite{solidity}. Ethereum Virtual Machine (EVM) is a stack-based virtual machine that executes the contract EVM bytecode.
The EVM executes transactions by splitting contract EVM bytecode into operation codes (opcodes), each with specific execution instructions.
% For example, the advertised ROI or the fee rate claimed in the DApp descriptions corresponds to the \textit{transfer} operations in the contract implementation.
% The total supply amount of the DApp token, which is critical for market stability and token scarcity~\cite{nftdefects}, is related to the mint functionality in the DApp contract.
% To ensure the stability of DeFi DApps, locking liquidity~\cite{liquidity} is proposed to offer
% a stable pricing environment and to encourage prolonged asset holding, as no one can withdraw their tokens from the liquidity pool~\cite{werner2022sok}.
% This functionality is also implemented in the contract function that determines the lock time.
% Furthermore, the accessibility of the NFT is reflected by the token URI which is set in the contract when minting NFTs.
% For example, the \textit{daily return 8\%} and the \textit{dev fee 5\%} shown in Figure~\ref{fig:description} correspond to the \textit{transfer} operations in contract implementation. The \textit{total supply} amount of the DApp token is related to the mint functionality in the DApp contract. Furthermore, the accessibility of NFT is reflected by the token URI which is set in the contract when minting NFTs.
% Ethereum Virtual Machine (EVM) is a stack-based virtual machine that executes the contract EVM bytecode.
% The EVM executes transactions by splitting contract EVM bytecode into operation codes (opcodes), each with specific execution instructions.
% However, the jump positions of EVM bytecode cannot be determined statically, and there are no return instructions for function call operations~\cite{chen2019large,nftdefects}.

\vspace{-0.2cm}
\subsection{Large Language Model}\label{sec:llmintro}
Recently, Large language models (LLMs) have exhibited remarkable proficiency in natural language understanding~\cite{icse24-llm}. 
Notably, ChatGPT~\cite{chen2023chatgpt} is distinguished by its advanced performance. However, it faces limitations such as limited availability in some regions and high API usage fees. 
%In contrast to closed-source models, the landscape of LLMs also includes open-source alternatives, exemplified by LLaMA~\cite{touvron2023llama}. 
%Despite the strong ability of ChatGPT, it is inaccessible in some countries and its price is high.
In contrast, LLaMA~\cite{touvron2023llama} offers advantages in terms of transparency, adaptability, cost-free access, and robust performance in natural language tasks. These features make LLaMA an ideal model for complicated or unstructured natural language understanding.
% Their self-supervised pre-training on vast datasets enables them to capture substantial domain knowledge without the need for task-specific data. This approach was pioneered by the GPT model in 2018~\cite{radford2018improving}, with subsequent models like GPT-3~\cite{brown2020language} and LLaMA~\cite{touvron2023llama} continuing to enhance LLM performance.
Additionally, the ability of LLaMA in downstream tasks can be further enhanced by its fine-tuning capabilities, a process of training the model on specific task-related labeled data in a supervised manner~\cite{devlin2018bert,liu2016recurrent}. This adaptability is further amplified in the context of instruction-tuning~\cite{zhang2023instruction,ouyang2022training,li2023tuna}, which trains models to interpret and act on explicit instructions in diverse tasks.
Numerous models have been developed based on LLaMA, including Code LLaMA~\cite{roziere2023code}, optimized for understanding and generating programming code, and LLaMA2~\cite{llama2}, which offers enhanced capabilities for natural language processing. Given our specific objective of comprehending intricate natural language data in DApp descriptions, we select LLaMA2 as our base model.

% For task-specific applications, LLMs undergo fine-tuning~\cite{devlin2018bert,liu2016recurrent}, a supervised process using labeled data that refines their performance on downstream tasks. Unlike full fine-tuning, the parameter efficient model fine-tuning (PEFT) approach~\cite{peft}, e.g., LORA~\cite{hu2021lora}, makes fine-tuning more affordable. This method enables efficient adaptation of pre-trained language models to various downstream applications without fine-tuning all the model's parameters but just adding tiny learnable parameters.
% To improve LLM's generalizability and adaptability across different domains and applications,
% instruction-tuning~\cite{zhang2023instruction,ouyang2022training,li2023tuna} trains models to interpret and act on explicit instructions in diverse tasks, employing diverse datasets loaded with instructions for more versatile task execution. 
% This method uses (\textit{INSTRUCTION}, \textit{OUTPUT}) pairs, where \textit{INSTRUCTION} denotes the human instruction for the model, and \textit{OUTPUT} represents the desired output that follows the \textit{INSTRUCTION}.


% \section{Motivation Example}
% In this section, we show a real-world DApp example to illustrate our motivation. 
% % DApp \textit{BNB Ultra} cheats users by hiding a fee-charging operation from the DApp descriptions, resulting in an unanticipated loss of user money.
% Figure~\ref{fig:bnbultra} shows the front-end description of DApp \textit{BNB Ultra}~\cite{bnbultra}.
% This DApp claims a ``3\% Daily Return'' and ``1,095\% APR'' on its description, which are related to the promised reward of users, trying to attract users' investment.
% However, the implementation of the DApp back-end smart contract has two inconsistencies with its description.
% First, the claimed return rate of 3\% is not guaranteed as the value of their eggs \verb|eggValue| (line 4 in Figure~\ref{fig:bnbultra}) are determined by \verb|marketEggs| and the contract balance (line 2), which are both undetermined variable factors, conflicting with the constant reward rate.
% Second, the contract shows a fee-charging logic (lines 7-9 in Figure~\ref{fig:bnbultra}), charging users a 6\% fee based on \verb|EggValue|, which is not shown in the DApp description, 
% % The inconsistency arises because the DApp's description does not show the fee rate but unanticipatedly charges users' fees in the contract code, 
% cheating users and hurting users' benefits.
% % The DApp description serves as a crucial conduit of information to potential users, which not only guides their understanding and usage of DApps but also exerts influence on their investment decisions by setting expectations for what the DApp can and cannot do.

% It is noticeable that this contract does not contain ``traditional'' vulnerabilities, e.g., \textit{reentrancy}, \textit{integer overflow}, which are covered by many academic and industrial tools~\cite{luu2016making,rao2012sailfish,choi2021smartian,liao2022smartdagger}. These two issues can only be detected by comparing the DApp description (\textit{say}) and the smart contracts implementation (\textit{do}).
% To fill this gap, in this paper, we first find what kind of inconsistencies exist in the DApp ecosystem and then uncover them by analyzing both DApp descriptions and contract implementation.

% \begin{figure}[htbp]
% \setlength{\abovecaptionskip}{0.cm}
% % \setlength{\belowcaptionskip}{-0.5cm}
%     \centering
%     \includegraphics[width=3.3in]{./images/background2.jpg}
%     \caption{DApp descriptions (top) and contract implementation snippet (bottom) of \textit{BNB Ultra}.}
%     \label{fig:bnbultra}
% \end{figure}
% \vspace{-0.5cm}

% \begin{figure}[htb]
% \setlength{\abovecaptionskip}{0.cm}
% \setlength{\belowcaptionskip}{-0.4cm}
% \begin{lstlisting}
% function calculateEggSell(uint256 eggs) public view returns(uint256){
%   return calculateTrade(eggs,marketEggs,address(this).balance);}
% function sellEggs() public {
%   uint256 eggValue=calculateEggSell(hasEggs);
%   uint256 baseFee=devFee(eggValue);
%   mrkoneAddress.transfer(baseFee*25/10); // 2.5%
%   mrktwoAddress.transfer(baseFee*25/10); // 2.5%
%   devAddress.transfer(baseFee*1); // 1%
%   msg.sender.transfer(SafeMath.sub(eggValue,baseFee*6));}
% \end{lstlisting}
% \caption{Hidden fee charging in BNB Ultra's contract.}
% \label{code:bnbultrafee}
% \end{figure}

% \subsection{DApp Front-end Description}
% Like traditional applications, a DApp's front-end description usually introduces its functionalities, features, and strengths~\cite{zhou2023dapphunter}. It serves as a crucial conduit of information to potential users, which not only guides their understanding and usage of DApps but also exerts influence on their investment decisions by setting expectations for what the DApp can and cannot do.
% % In order to attract users, DApps usually show the benefits they can provide and reveal the information related to the benefits of users using the DApp, e.g., daily return.

% Figure~\ref{fig:description} shows several examples of DApp descriptions. 
% The DApp \textit{Baked Onions} shows ``Daily Return 8\% ... Dev Fee 5\%'', claiming its mathematical information related to the reward of users and required fees of the DApp.
% The DApp \textit{BNB Tiger} says ``Total Supply ... Total Security ...'', showing the token information about the DApp's tokenomics.
% NFT DApp \textit{Cryptoz NFT Universe} declares that its NFT ``will live forever'' and ``are truly unique'', indicating the transparency of the token they provide.

% %In the area of DApps, where transactions can be irreversible and involve real assets, the front-end description provides information to potential users, guides their understanding and usage of DApps, influences their investment decisions, and sets expectations for what the dApp can and cannot do.

% \vspace{-0.3cm}
% \begin{figure}[htbp]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.5cm}
%     \centering
%     \includegraphics[width=3.3in]{./images/description.jpg}
%     \caption{Examples of DApp descriptions.}
%     \label{fig:description}
% \end{figure}
% \vspace{-0.2cm}

% \subsection{DApp Back-end Smart Contract}\label{bg:sc}
% The immutability of smart contracts ensures that their code and behavior cannot be modified once deployed; they are executed automatically according to the predefined logic~\cite{zheng2020overview}.
% Critical operations, such as the business logic of the DApp, are programmed in smart contracts.
% For example, the \textit{daily return 8\%} and the \textit{dev fee 5\%} shown in Figure~\ref{fig:description} correspond to the \textit{transfer} operations in contract implementation. The \textit{total supply} amount of the DApp token is related to the mint functionality in the DApp contract. Furthermore, the accessibility of NFT is reflected by the token URI which is set in the contract when minting NFTs.

% Previous works used texts in DApp UI widgets or buttons to analyze DApp intentions or business logic~\cite{duan2022towards,zhou2023dapphunter}, but they overlooked some descriptions. For example, none of the above-mentioned user assets-related information is concerned, which covers DApp information about users' reward, DApp tokenimics, etc. 
% It motivates us to analyze the DApp descriptions and find DApp inconsistencies to fill the gap.

==> icse2025-p517/03_definition.tex <==
\vspace{-0.2cm}
\section{Inconsistencies Definition}\label{sec:define}
%\subsection{Overview}
%This section illustrates how we define the seven types of DApp inconsistencies through a data collection and a data analysis process, as illustrated in Figure~\ref{fig:data}.
Figure~\ref{fig:data} illustrates how we define the seven types of DApp inconsistencies. First, we collected DApp descriptions and corresponding smart contracts from two platforms. Then, we employed the open card sorting approach~\cite{spencer2009card} to analyze the collected data manually. Finally, we defined seven DApp inconsistencies, each illustrated with a real-world DApp example.
%Then, we manually checked each of the collected DApps to find the inconsistencies between the DApps descriptions and smart contract implementation. Finally, we conducted a three-step classification based on the open card sorting approach~\cite{spencer2009card} to define seven DApp inconsistencies, and each of them is illustrated with a real-world DApp example.
% \vspace{-0.2cm}

\subsection{Data Collection}
% 表明收集的目的
% We first need to collect DApp descriptions and the corresponding smart contracts for manual inspection to identify and categorize inconsistencies.
% % 表明数据源的选择
% DappRadar~\cite{DappRadar} and DappBay~\cite{DappBay} are two major platforms that provide users with DApp websites and basic information about DApps (e.g., category, market cap, website, brief introduction, etc.).
% % 利用数据源做的事情
% Therefore, we obtained the front-end descriptions from the DApp websites provided by these two platforms and searched for smart contract addresses from the descriptions.
% % 最后收集的数量
% Finally, we collected the descriptions and corresponding contract addresses from \CollectedDApp~DApps, which serves as the data source to find and define DApp inconsistencies.

%Our data were collected from DappRadar~\cite{DappRadar} and DappBay~\cite{DappBay}, two main platforms that offer detailed information on DApps. 
We first crawled all \CollectedDApp~DApps labeled as \textit{high-risk} or \textit{red-alarm} by DappRadar~\cite{DappRadar} and DappBay~\cite{DappBay}, two main platforms that offer detailed information on DApps.
We then removed 255 DApps whose websites are inaccessible for further analysis and manually collected the HTML of each DApp by visiting their official websites. Next, we extracted related smart contract addresses from these websites and collected their source codes from Etherscan.
% can obtain the front-end descriptions from the DApp websites and search for smart contract addresses from the descriptions.
We finally obtained descriptions and smart contracts of 321 DApps. %This process yielded a dataset of \CollectedDApp~DApps, forming the basis for our analysis of DApp inconsistencies.

\vspace{-0.3cm}
\begin{figure}[htbp!]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=3.3in]{./images/data1.png}
    \caption{Workflow of defining DApp inconsistencies.}
    \label{fig:data}
\end{figure}

\vspace{-0.3cm}
\subsection{Data Analysis}\label{sec:opencardsoring}
% 收集数据后打算做什么
% Following the data collection phase, 
% It is noticeable that the inconsistency exists if one of the four cases
%To ensure the correctness of the analysis results, we 

To find DApp inconsistencies, three authors use the open card sorting approach~\cite{spencer2009card}, which is widely adopted in problem-finding and definition in software engineering~\cite{nftdefects,chen2020defining}.
% 表明关注的属性（user关注的，与收益或资产相关的）
% In this process, we first read the descriptions on the DApp and find those related to the smart contract implementations (e.g., profit given to users or fee charged from users). We mainly focus on those highly related to the users' profits or assets as they are the first concerns for users.
% 首先需要定义aim，然后在部分数据上进行一轮card sorting
% 前后端分别作post，然后提出关注的内容做比对(fund-related)
% 需要说明第一轮sorting需要大概列出关注的一些属性
In this process, we first created a card that contains the front-end description and the contract code for each DApp. We considered two aspects to ensure the significance of the inconsistency issues, namely user financial-related information in DApp descriptions (e.g., promised return on investment, claimed fees charged, and the stability of the token economy) and corresponding financial-related code logic in smart contract implementations. These aspects are highly related to users' profits or assets and are usually the major concern of users. Then, three authors worked together to determine the labels for each card. They followed the detailed steps illustrated in the previous problem definition works~\cite{nftdefects,chen2020defining}.

% 具体步骤，先读前端文本，找关键信息
There are three steps in the open card sorting process. In the first step, they randomly chose 40\% of the cards and read the DApp descriptions. They extracted the claims that are related to users' funds or assets, e.g., \textit{our DApp pays 8\% daily for users}, or \textit{we charge another 4\% fee for marketing}, etc.
% 合约理解，同样找关键信息
Similarly, they read the contract code and focused on the implementations related to the fund transfer or tokens. They checked the transfer target, the transfer amount, and other attributes related to the assets. 
For those contracts without source code, they used an online decompiler~\cite{Dedaub} and analyzed the contract IR.
% 通过比较得到不一致
Based on the two aspects of information extracted from the DApp description and the smart contract, they compared them and understood the inconsistencies.

In the second step of card sorting, the same three authors analyzed and categorized the remaining 60\% cards independently, following the same steps as in the first round. 
Meanwhile, if they encountered new descriptions or contract implementation related to users' funds or assets other than what they found in the first round (e.g., daily reward), they kept the cards to the final discussion.


In the third step, they compared the results, discussed the differences, and finally identified seven types of inconsistencies across \DAppGT~DApps from all the collected \CollectedDApp~DApps. The remaining 267 DApps found no further inconsistencies or had no financial-related codes or descriptions during the open card sorting process.
% They filtered \DAppGT~DApps with their inconsistency labels from all the collected \CollectedDApp~DApps and
We established the mapping relationship between the filtered DApp and the defined inconsistencies, which is publicly available in our repository.
%Users can be confused by the DApps and lose money due to those inconsistencies.

% \vspace{-0.5cm}
\subsection{Definition of DApp Inconsistencies}
Table~\ref{tab:inconsistency} shows the definition of seven inconsistency types between the DApp front-end descriptions and smart contracts. The third column highlights the inconsistency types, and to clearly show each inconsistency, we list both the illustration of front-end descriptions and the implementation of smart contracts (columns fourth and fifth). Our defined inconsistencies cover NFT and DeFi DApps.
% 下面这一段表达可以更简洁一点
% In our paper, there are two scenarios of inconsistency. (1) The front-end description claims behavior A with attribute x, and this behavior is implemented in the contract, but the attribute is y, while x != y. For example, the DApp claims to charge a 3\% fee for development, while the contract actually charges 5\%. The fee transfer behavior is mentioned in both the description and the contract, but the attribute value is inconsistent.
% (2) The DApp description does not reveal the behaviors the contract does. For instance, the contract charges fees from users, but the fee rate is not mentioned on the DApp front-end.

The following paragraphs provide the corresponding detailed definition and example for each inconsistency.

\begin{table*}[htbp]
\setlength\tabcolsep{3pt}
    \setlength{\abovecaptionskip}{-0.5cm}
    \setlength{\belowcaptionskip}{-0.7cm}
    \begin{center}
        \caption{Definitions of the 7 DApp Inconsistencies.}
        \label{tab:inconsistency}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{General Type}                  & \textbf{DApp Type}                 & \textbf{Inconsistency Type}  & \textbf{Front-end Description}                                               & \textbf{Smart Contract Implementation}                           \\ \hline
\multirow{2}{*}{Mathematics}  & \multirow{3}{*}{DeFi}     & \textit{Unguaranteed Reward (UR)}              & Claim a reward of x\%                                               & Reward rate is not a guaranteed constant value                     \\ \cline{3-5} 
                              &                           & \textit{Hidden Fee (HF)}                 & Not claim fee or claim fee as x\%                                & Fees are charged with a rate of y\% (y!=x)                    \\ \cline{1-1} \cline{3-5} 
\multirow{5}{*}{Transparency}  &                           & \textit{Adjustable Liquidity (AL)}        & Claim x years of liquidity lock time                                           & The lock time are adjustable to be less than x                      \\ \cline{2-5} 
                              & \multirow{3}{*}{DeFi/NFT} & \textit{Unconstrained Token Supply (UTS)} & Claim a token supply of x                                &    The supply can be bigger than x                        \\\cline{3-5}  &                           & \textit{Unclaimed Fund Flow (UFF)}           & Not claim the possible fund flow to the project owner            & The contract fund can be withdrawn by specific users \\ \cline{3-5} 
                              &                           & \textit{Changeable DApp Status (CDS)}         & Not claim the possible pause of the DApp                         & The DApp can be paused to impede trading                \\ \cline{2-5} 
                              & NFT                       & \textit{Volatile NFT Accessibility (VNA)}   & Not claim the accessibility of NFTs or claim they are accessible & The NFTs can be inaccessible                            \\ \hline

\end{tabular}%
}
\end{center}
\vspace{-0.4cm}
\end{table*}

\textbf{(1) Unguaranteed Reward (UR):}
Rewards are pivotal in incentivizing user investment in DApps.
Some DApps advertise high rewards to attract investments, but inconsistencies between these advertised rewards and the contract's actual implementation can deceive users. Such inconsistencies might lead to users not receiving the guaranteed rewards or even resulting in financial loss.
% In order to attract users, DApps can claim a high reward trying to gather more users' investment. 
% If the contract implementation is inconsistent with the claim in the description, users can be deceived by DApps, which can gather assets to pull the rug. As a consequence, users may not receive the claimed reward or even lose all of the investment.

\vspace{-0.3cm}
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.3cm}
    \centering
    \includegraphics[width=3.3in]{./images/background3.jpg}
    \caption{DApp descriptions (top) and contract snippet (bottom) of \textit{BNB Ultra}.}
    \label{fig:reward}
\end{figure}
\vspace{-0.1cm}

\textbf{Example:} Descriptions on \textit{BNB Ultra}~\cite{bnbultra} (Figure~\ref{fig:reward}) might mislead users that they can obtain a daily profit of 3\%. % for users. However, this claim is misleading due to the qualifier ``according to the current mining efficiency rate.'' 
An examination of the contract~\cite{bnbultracontract} reveals that the reward is not guaranteed. 
Specifically, line 9 indicates that the user reward comprises two components, i.e., the value of \textit{eggs} and \textit{baseFee}. The value of \textit{eggs} is determined by the function \textit{calculateTrade()} (line 2), depending on variable \verb|marketEggs| and contract balance. This implementation means that the promised 3\% reward rate is subject to undetermined variable factors, contradicting the front-end claim.


% Figure~\ref{fig:reward} is the front-end description of the DApp \textit{BNB Pirates}, which provides users 3\% daily profit. 
% The constant numeric value 3\% is misleading, as the following description shows ``accroding to the current mining efficiency rate''.
% However, as we read the contract, we find that the 3\% profit promised to the users is not guaranteed. Figure~\ref{code:reward} shows the contract implementation of the reward transfer to users (lines 6-17). From line 17, the reward of users can be divided into two parts, i.e., the value of eggs (denoted by variable \verb|eggValue|) and the fees (denoted by \verb|fee|). However, the value of the investment ``egg" is calculated by the formula implemented in the function \textit{calculateTrade()} (line 3), which is obtained by the undetermined variable \verb|marketEggs| and the contract balance (by \verb|balanceOf(address(this)|).
% The claimed misleading constant reward rate of 3\% is inconsistent with the implementation of the contract, making the reward subject to undetermined variables.

% \vspace{-0.2cm}
% \begin{figure}[htb]
% \setlength{\abovecaptionskip}{0.cm}
% \setlength{\belowcaptionskip}{-0.4cm}
% \begin{lstlisting}
% function calculateEggSell(uint256 eggs) public view returns(uint256){
%   return calculateTrade(eggs,marketEggs,address(this).balance);}
% function sellEggs() public{
%   uint256 eggValue=calculateEggSell(hasEggs);
%   uint256 baseFee=devFee(eggValue);
%   mrkoneAddress.transfer(baseFee*25/10); // 2.5%
%   mrktwoAddress.transfer(baseFee*25/10); // 2.5%
%   devAddress.transfer(baseFee*1); // 1%
%   msg.sender.transfer(SafeMath.sub(eggValue,baseFee*6));}
% \end{lstlisting}
% \caption{Contract code snippet of \textit{BNB Pirates}.}
% \label{code:reward}
% \end{figure}

\vspace{-0.3cm}
\begin{figure}[!htbp]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=3.3in]{./images/supply.jpg}
    \caption{DApp description (top) and contract snippet (bottom) of \textit{MILKY} token.}
    \label{fig:supply}
\end{figure}
\vspace{-0.3cm}

\textbf{(2) Hidden Fee (HF):}
DApps often charge fees to maintain their operations, compensating for resources such as management efforts. However, issues arise when these fees are either undisclosed on the DApp's front-end description or differ from the actual contract implementation, which can unexpectedly impact user assets and compromise the DApp's trustworthiness.

% To cover the operational costs associated with the execution and maintenance of the project, DApps usually charge users fees. These fees ensure that DApp developers and maintainers are compensated for the resources they allocate, including computational power, storage, and the overall management of the DApp. However, if fees are silently charged (fees are not claimed on the DApp website), or the claimed charged fees are inconsistent with the contract implementation, the assets of the users can be unexpectedly influenced, and the trustworthiness of the DApp can be ruined.

\textbf{Example:} 
Returning to \textit{BNB Ultra}~\cite{bnbultra}, the final reward for users is reduced by fees directed to predetermined addresses (Figure~\ref{fig:reward}, line 9). Specifically, lines 6-8 show fees being allocated to three different addresses, with the total fee amount determined by the \textit{devFee()} function (line 5). However, this fee structure~\cite{bnbultracontract} is not disclosed in the DApp’s front-end description (Figure~\ref{fig:reward}), resulting in a \textit{Hidden Fee} inconsistency. %Additionally, DApp \textit{Block Reward} claims a development fee as 1\% in the DApp description~\cite{bpblockreward} but implements it as 6\%~\cite{blockrewardcontract}, cheating DApp users.
% As we mentioned in \textit{Reward Inconsistency} of \textit{BNB Pirates}, the final reward transferred to users is subtracted by fees transferred to some constant addresses set by the DApp owner, as shown in Figure~\ref{code:reward} (line 17). Specifically, fees are charged by \verb|ceoAddress|, \verb|ceoAddress2|, and \verb|ceoAddress3| (lines 14-16). The total amount of the fee charged is calculated using the function \textit{devFee()} (line 10). However, the DApp does not mention the charged fees or claims how the fees are distributed in the description shown in Figure~\ref{fig:reward}, leading to inconsistency.
% Additionaly, 是不是可以放一个说了fee但是数值不一致的case

\textbf{(3) Unconstrained Token Supply (UTS):}
Many DApps have their native tokens, e.g., Aave~\cite{aave} and BAYC~\cite{bayc}. Setting the maximum supply of tokens can uphold tokens scarcity~\cite{nftdefects}, stabilizing the market.
% However, if the token supply is inconsistent with the amount claimed, holders should be harmed due to the increase in the price of the token supply and the impact of scarcity~\cite{brekke_digital_2021}.
Inconsistencies between the stated token supply and actual contract code can detrimentally affect token holders by affecting the token's value and scarcity~\cite{brekke_digital_2021}.

% \vspace{-0.3cm}


\textbf{Example:}
% Figure~\ref{fig:supply} shows a front-end description of the total supply of the \textit{MILKY} token. The claimed total supply is a constant value of 250,000,000. However, the contract code shown in Figure~\ref{code:supply} can make the total supply exceed the claimed amount.
% Specifically, the contract owner can directly skip the \textit{onlyOwner} modifier to mint tokens, which have no supply amount restriction. The value of the token can be threatened if there is an inconsistency that cheats users.
Descriptions about the \textit{MILKY} token~\cite{bpmliky} claims a total supply of 250M (Figure~\ref{fig:supply}). However, the contract~\cite{mlikycontract} (line 2) allows one to mint tokens without a supply cap. %This inconsistency could devalue the token~\cite{nftdefects} and pose threats to users.

% \vspace{-0.cm}
% \begin{figure}[htb]
% \setlength{\abovecaptionskip}{0.cm}
% \setlength{\belowcaptionskip}{-0.1cm}
% \begin{lstlisting}
% function mint(uint256 amount) public onlyOwner returns (bool) {
%   _mint(_msgSender(), amount);
%   return true;}
% function _mint(address account, uint256 amount) internal {...
%   _totalSupply = _totalSupply.add(amount);
%   _balances[account] = _balances[account].add(amount);}
% \end{lstlisting}
% \caption{Contract code snippet of \textit{MILKY} token.}
% \label{code:supply}
% \end{figure}
% \vspace{-0.3cm}

\textbf{(4) Adjustable Liquidity (AL):}
% The liquidity lock time of DeFi DApps is a great indicator to show DApp stability~\cite{liquidity}. First, locking liquidity can provide a more stable pricing environment, therefore, bolstering market confidence. Second, with liquidity locked, investors are more inclined to hold their assets longer. However, if the liquidity lock time is not consistent with the DApp claims or can be arbitrarily changed, there will be unstable inflows and outflows in the market, inducing market panic, and leading to a price drop, which will harm the holders' benefits.
Liquidity lock time refers to a period during which some users (e.g., token project managers) cannot withdraw their tokens.
The liquidity lock time in DeFi DApps is crucial for stability~\cite{liquidity}, offering a stable pricing environment and encouraging prolonged asset holding. Inconsistencies in this aspect, such as unaligned claims or adjustable lock times, may cause market instability and compromise the interests of investors.


\vspace{-0.3cm}
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{-0.1cm}
% \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    \includegraphics[width=3.3in]{./images/lock1.jpg}
    \caption{Description (top) and contract snippet (bottom) of \textit{Baby BNB Tiger}.}
    \label{fig:lock}
\end{figure}
\vspace{-0.2cm}

\textbf{Example:}
% Figure~\ref{fig:lock} shows the token information of the DApp \textit{BNB Tiger}. It says that the DApp's liquidity is locked up for 5 years. However, its smart contract shown in Figure~\ref{code:lock} makes this lock time modifiable. The function \textit{lock()} (lines 1 to 4) can be called by the owner to set any time they want through the unconstrained parameter \verb|time|, and there is no constraint on the time to ensure the claimed ``5 year" duration.
% This issue can make the liquidity lock time not a constant value, as the DApp front-end description claims, leading to inconsistency. 
\textit{Baby BNB Tiger} claims a 5-year liquidity lock~\cite{bpbabytiger} (Figure~\ref{fig:lock}). However, its contract~\cite{babytigercontract} allows the owner to modify this time (line 4) through the \textit{lock()} function arbitrarily. %This flexibility contradicts the front-end claim and introduces potential inconsistencies, impacting market stability and DApp trustworthiness.

% \vspace{-0.2cm}
% \begin{figure}[htb]
% \setlength{\abovecaptionskip}{0.cm}
% \begin{lstlisting}
% function lock(uint256 time) public virtual onlyOwner {
%   _previousOwner = _owner;
%   _owner = address(0);
%   _lockTime = block.timestamp + time;}
% \end{lstlisting}
% \caption{Contract code snippet of \textit{Baby BNB Tiger}.}
% \label{code:lock}
% \end{figure}
% \vspace{-0.2cm}
% function unlock() public virtual {
%     require(_previousOwner == msg.sender, "You don't have permission to unlock");
%     require(block.timestamp > _lockTime , "Contract is locked until 7 days");
%     _owner = _previousOwner;}


\textbf{(5) Unclaimed Fund Flow (UFF):}
% Funds are an important concern for users when using DApps. Users deposit or transfer funds to DApp contracts in order to make profits. In some cases, DApp developers retain the ability to make an emergency withdrawal to protect user assets when they find DApp bugs or upgrade their contract for security. However, if they do not make this information open and give clear reasons to gain users' trust, but maliciously keep the privileged withdrawal function, the DApp users' assets can be exposed to high risk, which could cause a ripple effect that users become wary of other DApps as well, therefore damaging the trust between users and DApps.
%Funds management is a crucial aspect for users in DApps, where they deposit funds with the expectation of profit.
Most DApps allow users to deposit or transfer funds to make profits. In some cases,  
DApp owners may have the capability for emergency withdrawals. However, transparency is important for users.  Failure to disclose this capability can significantly risk user assets~\cite{fundtransfer} and lead to a loss of trust in the DApp ecosystem. %Such actions not only affect individual DApps but could also make users cautious of other DApps, undermining overall user confidence.

\textbf{Example:}
% The DApp \textit{Metarevo} does not claim any possible fund flow to the project owner or the permission control to operate fund withdrawal, e.g., multi-signature wallet or DAO. However, its back-end contract does. As shown in Figure~\ref{code:clear}, all the contract balance can be withdrawn by the owner (line 8) through the function \textit{clearETH()} (lines 5 to 8). The permission control in line 6 can be skipped by setting \verb|_authNum| by the owner (line 3).
The DApp \textit{Metarevo}~\cite{bpmetarevo} (Figure~\ref{code:clear}) does not disclose that the owners have the ability to transfer users' assets in front-end descriptions. However, its contract~\cite{metarevocontract} allows the owner to withdraw all balances (line 8) via the \textit{clearETH()} function (lines 5-8).%, bypassing permission controls by adjusting \verb|_authNum| (line 3), which can expose user assets to risks and erode trust in DApps.

\vspace{-0.3cm}
\begin{figure}[htb]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.6cm}
\begin{lstlisting}
function authNum(uint256 num)public returns(bool){
    require(_msgSender() == _auth, "Permission denied");
    _authNum = num;
    return true;}
function clearETH() public onlyOwner() {
    require(_authNum==1000, "Permission denied");
    _authNum=0;
    msg.sender.transfer(address(this).balance);}
\end{lstlisting}
\caption{Contract code snippet of \textit{Metarevo}.}
\label{code:clear}
\end{figure}
\vspace{-0.3cm}

% \vspace{-0.3cm}
% \begin{figure}[htb]
% \setlength{\abovecaptionskip}{0cm}
% \setlength{\belowcaptionskip}{-0.6cm}
% \begin{lstlisting}
% function authNum(uint256 num)public returns(bool){
%     require(_msgSender() == _auth, "Permission denied");
%     _authNum = num;
%     return true;}
% function clearETH() public onlyOwner() {
%     require(_authNum==1000, "Permission denied");
%     _authNum=0;
%     msg.sender.transfer(address(this).balance);}
% \end{lstlisting}
% \caption{Contract code snippet of \textit{Metarevo}.}
% \label{code:clear}
% \end{figure}
    

\textbf{(6) Changeable DApp Status (CDS):}
% Pause functionality provides developers with an approach to prepare for unexpected events or necessary intervention~\cite{pause}. 
% For example, when finding bugs in their codes, DApp developers can pause the DApp to prevent potential exploits or loss of user funds.
% Also, when there is an upgrade of the smart contract, the DApp should be paused to ensure that no transactions occur that might conflict with the update.
% However, if users do not get the information, such as whether the DApp can be or has been paused or the historical pause information, their transactions, including trading, can be reverted. This inconsistency can undermine the trust of users towards the DApp with unexpected bad user experience.
% Therefore, it is important for developers to clearly expose this information to users about the reasons and conditions under which the pause function might be used.
The pause function in DApps provides developers with the capability to manage unexpected events (security issues) or implement updates~\cite{pause}. %This function is crucial to prevent potential exploits or transaction conflicts during updates. 
However, the lack of information about the pause status for users may result in failed transfers, eroding trust in the DApp.
%It's essential for developers to clearly demonstrate the reasons and conditions for using the pause function to users if they support pause functionality.

\textbf{Example:}
% Figure~\ref{code:pause} shows the pause operation in the smart contract of DApp \textit{BalanceNetWork}, which does not claim its feature of pausing the DApp to stop token trading. Specifically, the function \textit{pause()} (lines 1 to 3) enables the owner to pause the DApp. However, the DApp pause will stop the trading system. The token transfer cannot be executed as the modifier \textit{whenNotPaused} restricts the function \textit{\_transfer()}. As the DApp does not claim why and how the DApp can be paused, the DApp status inconsistency can influence the users.
In the \textit{BalanceNetWork} DApp~\cite{bpbalancenetwork}, the pause functionality is not publicly disclosed (Figure~\ref{code:pause}). The \textit{pause()} function (lines 1-3) allows the owner to pause the DApp~\cite{balancenetworkcontract}, which stops the trading system by restricting the \textit{\_transfer()} function (lines 4-7) by \textit{whenNotPaused} modifier. %The absence of clarity on why and how the DApp can be paused introduces inconsistencies can negatively impact users.

\vspace{-0.4cm}
\begin{figure}[htb]
\setlength{\belowcaptionskip}{-0.4cm}
\setlength{\abovecaptionskip}{-0.1cm}
\begin{lstlisting}
function pause() onlyOwner whenNotPaused external {
    paused = true;
    emit Pause();}
function _transfer(address from, address to, uint256 value) internal whenNotPaused {
    ...
    _balances[from] -= value;
    _balances[to] += value;}
\end{lstlisting}
\caption{Contract code snippet of \textit{BalanceNetWork}.}
\label{code:pause}
\end{figure}
\vspace{-0.3cm}

\textbf{(7) Volatile NFT Accessibility (VNA):}
% NFTs (Non-fungible tokens) represent digital ownership of unique assets on the blockchain, serving as verifiable proof ownership~\cite{nftdefects}. 
% This ownership is detailed and enriched by metadata, which provides information about the digital assets the NFTs stand for. When the metadata is stored on centralized servers, such as HTTPS~\cite{HTTPS2023}, it introduces problems, since assets on centralized systems can become inaccessible if the server faces shutdowns or other issues~\cite{das2022understanding}, contradicting the longevity and permanence that blockchains promise. 
% Despite the decentralized nature of NFTs, storing their metadata in a centralized manner introduces an inconsistency. 
% If a DApp professes that its NFTs ``live forever on the blockchain'' but then opts for centralized storage for its metadata, it undermines the core value proposition of enduring accessibility. For genuine durability and consistency, decentralized storage solutions, such as IPFS, are strongly recommended for NFT metadata~\cite{das2022understanding}.
NFTs represent digital ownership of unique assets on the blockchain~\cite{nftdefects}. However, storing NFT metadata on centralized servers while claiming its permanence introduces inconsistencies. Centralized storage is susceptible to shutdowns or issues~\cite{das2022understanding}, conflicting with the promise of permanence and longevity.
To ensure durability, decentralized solutions such as IPFS~\cite{ipfs} and Arweave~\cite{arweave} are recommended for storing NFT metadata.

\vspace{-0.2cm}
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.3cm}
    \centering
    \includegraphics[width=3.3in]{./images/nft1.jpg}
    \caption{Description (top) and contract snippet (bottom) of \textit{Cryptoz Universe}.}
    \label{fig:nft}
\end{figure}
% \vspace{-0.3cm}

\textbf{Example:}
\textit{Cryptoz Universe NFT} claims its NFTs can live forever on the blockchain~\cite{bpcryptoz} (Figure~\ref{fig:nft}). However, its smart contract~\cite{cryptozcontract} uses HTTPS for metadata storage (line 1). When this server was shut down, the NFTs became inaccessible, hurting user benefits and contradicting the claim of permanence.

% \vspace{-0.3cm}
% \begin{figure}[htb]
% \setlength{\abovecaptionskip}{0.cm}
% \setlength{\belowcaptionskip}{-0.5cm}
% \begin{lstlisting}
% string baseTokenURI = "https://cryptoz.cards/data/";
% function tokenURI(uint256 _tokenId) external view returns (string memory) {
%   return Strings.strConcat(baseTokenURI, Strings.uint2str(_tokenId));}
% \end{lstlisting}
% \caption{Contract code snippet of \textit{Cryptoz Universe NFT}.}
% \label{code:nft}
% \end{figure}


==> icse2025-p517/04_method.tex <==
\vspace{-0.2cm}
\section{Methodology}
In this section, we introduce our tool \textsc{Hyperion}, which is capable of detecting the seven types of inconsistencies defined above by analyzing DApp descriptions and smart contracts.
% We first give an overview of our approach and then illustrate the details of the LLM-based DApp description analysis and the contract semantic analysis with dataflow-driven symbolic execution, respectively.
%This section outlines our tool, \textsc{Hyperion}, designed to detect the 7 types of DApp inconsistencies by analyzing their descriptions and smart contracts. We provide an overview of our approach, followed by details on DApp description analysis using an LLM and contract semantic analysis through dataflow-guided symbolic execution.

\vspace{-0.2cm}
\subsection{Overview}
Figure~\ref{fig:overview} shows an overview of the \textsc{Hyperion}, which has three components, namely \textit{Description Analysis}, \textit{Contract Semantic Analysis}, and \textit{Inconsistency Detection}.

\vspace{-0.1cm}
\begin{figure}[hbtp]
    \setlength{\abovecaptionskip}{-0.4cm}
    % \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=\linewidth]{./images/overview.jpg}
    \caption{Overview of \textsc{Hyperion} approach.} \label{fig:overview}
\end{figure}
\vspace{-0.3cm}


% % 前端分析
% Specifically, users need to input an accessible DApp URL, a DApp HTML file or a txt file containing DApp descriptions, and the smart contract address. For description analysis, the DApp description will be fed into our fine-tuned LLaMA2 model with a designed prompt template (see Section~\ref{sec:llm}), and the LLM output will be further processed using our inconsistency-related attribute extraction method based on the Natural Language Tool Kit~\cite{nltk} (NLTK).
%\textsc{Hyperion} comprises three key components, i.e., \textit{Description Analysis}, \textit{Contract Semantic Analysis}, and \textit{Inconsistency Detection} (Figure~\ref{fig:overview}). 
The input of \textsc{Hyperion} contains two parts, i.e., front-end description (can be a DApp URL, HTML, or text) and back-end contract code. 

For \textit{Description Analysis}, the DApp descriptions are first parsed as raw text, and then concatenated with our designed prompts through \textsc{HyperText}, which is obtained by LLaMA2 instruction-tuning (see Section~\ref{sec:fine-tune}). Next, NLTK is employed to extract inconsistency-related attributes from the output of \textsc{HyperText} (LLM responses), which are used for further comparison with the contract semantics.% and further analyzed by an attribute extraction method based on NLTK.

% 后端分析
% For contract semantic analysis, the input contract address will be used to obtain the contract bytecode through the Web3 API~\cite{web3py}. Then the bytecode will be compiled by Elipmoc~\cite{grech2022elipmoc}, a widely used decompiler that can recover an intermediate representation (IR) for the EVM bytecode and supports declarative dataflow rule programming on this IR. 
% Next, \textsc{Hyperion} performs a dataflow analysis on this IR and recovers the inconsistency-related semantics, e.g., fund transfer. We use recovered semantics to construct two graphs, i.e., fund transfer graph and the storage variable dependency graph, to obtain higher-level features and guide our targeted symbolic execution on the IR.
% Our dataflow-driven symbolic execution on this IR helps us aimly trace the inconsistency-related path, and the SMT solve helps us validate the program states and find contract semantics.
% Finally, according to the inconsistency-related attributes extracted from the DApp description and contract semantics recovered from program analysis, \textsc{Hyperion} identifies the inconsistency based on the detection rules.
In \textit{Contract Semantic Analysis}, \textsc{HyperCode} first decompiles the contract bytecode using Elipmoc~\cite{grech2022elipmoc}, to recover the CFG and the contract IR. \textsc{HyperCode} then performs dataflow analysis on this IR to extract inconsistency-related semantics, such as fund transfers. This analysis includes constructing fund transfer and storage variable dependency graphs that guide targeted symbolic execution on the IR to trace inconsistency-related paths. Furthermore, the SMT solver validates program states collaborated with on-chain state extraction, thus identifying contract semantics.

Finally, in \textit{Inconsistency Detection}, \textsc{Hyperion} incorporates the attributes extracted from DApp descriptions and contract semantics to identify inconsistencies based on defined rules.

% \textsc{Hyperion} fine-tunes an LLM to understand the description, as the front-end texts are diverse, while the LLM is well performed in complex natural language understanding. In fact, we designed prompts and fine-tuned the LLM with multiple experiments, making it a domain-specific ``expert'' in understanding the descriptions of the DApp.
% Furthermore, the IR is used in the symbolic execution of the EVM bytecode for the first time, as far as we are concerned. We designed this symbolic execution module as an extensible framework for users to program more rules on it.
%This approach utilizes the LLM's natural language understanding capabilities for diverse front-end texts, transforming it into a domain-specific tool for analyzing DApp descriptions. Additionally, the use of contract IR-based symbolic execution is a novel aspect of our methodology, providing an extensible framework for programming additional analysis rules.

% The IR-based control flow graph (CFG) is complete, making it possible to trace some specific basic blocks, reducing the execution time, while traditional symbolic executors require full execution to find the jump target of some basic blocks.

\subsection{LLM-based DApp Description Analysis} \label{sec:llm}
In this subsection, we give details of how we extract attributes related to inconsistencies from the DApp description. % Then, in Figure~\ref{fig:nltk}, we illustrate the workflow of \textsc{HyperText} with parsing the DApp HTML file into raw text, which is then concatenated with our designed prompts. After feeding the combined input to \textsc{HyperText}, NLTK is employed for extracting inconsistency-related attributes, which are used for inconsistency detection.

% \begin{figure}[!hbtp]
%     \setlength{\abovecaptionskip}{0.cm}
%     \setlength{\belowcaptionskip}{-0.5cm}
%     \centering
%     \includegraphics[width=3.3in]{./images/nltk.png}
%     \caption{Workflow of \textsc{HyperText}.} \label{fig:nltk}
% \end{figure}% through the LLM and NLTK.
% 为什么要选择llama
%We adopt LLaMA2 as our base model (see Section~\ref{sec:llmintro}) %The main reason we do not choose ChatGPT is due to its inaccessibility in some countries and its high price.
% We have chosen the LLaMA2-13b-chat model for our analysis. The main reason we do not choose ChatGPT~\cite{bahrini2023chatgpt} is due to its inaccessibility in some countries and its high price.
% This particular version of LLaMA2 is selected for its balance between performance and resource consumption. While smaller LLaMA models like the 7b parameter version offer less computational load, they do not match the 13b model in effectiveness. On the other hand, larger models, such as the 70b parameter version, require significantly more resources and may not be feasible for our server capabilities.
% A key aspect of our methodology is the parameter setting during model inference. We set the parameter \textit{do\_sample} as false to eliminate randomness in the LLM's output. This approach ensures consistent and reliable analysis, vital for accurately extracting data from DApp descriptions.

% This subsection outlines our approach for extracting inconsistency-related attributes from DApp descriptions using the LLaMA2-13b-chat model. We selected LLaMA2-13b-chat~\cite{MetallamaLlama213bchathfHugging} for its balance of performance and resource efficiency. Although the smaller 7b version is less resource-intensive, it falls short in effectiveness compared to the 13b model. Conversely, the larger 70b model, while more powerful, is demanding server resources.
% We do not choose ChatGPT~\cite{bahrini2023chatgpt} due to its inaccessibility in some countries and its high price. A crucial component of our approach is ensuring consistent and reliable outputs from the LLM. To achieve this, we set the \textit{do\_sample} parameter to false during model inference, eliminating randomness in the LLM's output. This strategy is pivotal for accurate and dependable extraction of data from DApp descriptions.

% subsection details our methodology for extracting attributes related to inconsistencies from DApp descriptions, employing the LLaMA2-13b-chat model. Chosen for its optimal balance between performance and resource usage, the LLaMA2-13b-chat model~\cite{MetallamaLlama213bchathfHugging} outperforms its less resource-intensive 7b counterpart and is more feasible than the more demanding 70b version. We opted against ChatGPT~\cite{bahrini2023chatgpt} due to accessibility constraints and cost considerations.
% \vspace{-0.2cm}

\subsubsection{Instruction-Tuning}\label{sec:fine-tune}
In this part, We introduce the process of obtaining our \textsc{HyperText} model. We adopt LLaMA2 as our base model due to its adaptability, cost-free access, and excellent performance in natural language tasks (see Section~\ref{sec:llmintro}). To make LLaMA2 perform well in our downstream DApp description analysis task, we propose an instruction-tuning approach, as depicted in Figure~\ref{fig:llm_overview}.
Specifically, after we obtain the raw text of the description, (1) we first design specific prompts to improve the model's efficacy in yielding the specific desired attributes we want to extract. (2) Next, we adopt a prompt segmentation method to fix issues caused by long input. (3) Then, we perform instruction tuning with manually labeled DApp descriptions and finally get our model \textsc{HyperText}.

\begin{figure}[hbtp]
    \setlength{\abovecaptionskip}{-0.1cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=3.3in]{./images/llm_ft.jpg}
    \caption{Workflow of LLaMA2 Instruction-Tuning.} \label{fig:llm_overview}
\end{figure}
\vspace{-0.3cm}
% , our analysis process begins with data preprocessing to prepare LLaMA2's input text. We then utilize specifically designed prompts to maximize the efficacy of the model. The LLaMA2 is further refined through fine-tuning with labeled descriptions, enhancing its capability for the downstream DApp description analysis. Finally, we employ NLTK to precisely extract key attributes and structure the LLaMA2’s output.

% Figure~\ref{fig:llm_overview} shows an overview of how we analyze the description. We first perform data preprocessing to obtain the input raw text of LLaMA2; then, we use designed prompts to make full use of LLM. Furthermore, we fine-tune the LLM via labeled description with rectified expected output, making the LLM more applicable to the downstream DApp description analysis task.
% Finally, we employ the NLTK to extract essential attributes and structure the output from the LLM.


% 训练和推理拆分
% ft stage + infer stage

% raw text + prompt design
% 新模型

% infer
% raw text 给自己的模型+NLTK

\vspace{-0.3cm}
\begin{figure}[hbtp]
    \setlength{\abovecaptionskip}{-0.4cm}
    % \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=\linewidth]{./images/numeric2.png}
    \caption{Prompt Template of Numeric Inconsistency-related Information.} \label{fig:numeric}
\end{figure}

% prompt的选择，以及token的选择
\para{Prompt Design}\label{sec:promptdesign}
LLMs operate on a prompt-based learning approach~\cite{prompt}, with prompt design crucially impacting performance~\cite{chen2023chatgpt}. We adopt LLaMA2's recommended prompt structure~\cite{llama2prompt}, comprising a system prompt ($SP$) and a user prompt ($UP$).
% The $SP$ includes the designated model's role $R$ and general instructions $GI$.
% We define $R$ as the \textit{expert in blockchain and smart contracts}, aligning with the seven inconsistencies we aim to detect, and incorporate $GI$ for clarity and accuracy, such as \textit{avoiding false information sharing}.
$SP$ defines the model's role $R$, e.g., requiring the model to act as a \textit{``smart contract expert''} and includes general instructions $GI$ to ensure accuracy, e.g., requiring the model to \textit{``avoid sharing false information''}.
The user prompt $UP$ is divided into $UP_{it}$ and chain of thought~\cite{wei2023chainofthought} ($UP_{CoT}$) components.
Specifically, $UP_{it}$ directs LLM to analyze and extract specific kinds of inconsistency-related information types, i.e., numeric and boolean. 
Figure~\ref{fig:numeric} and Figure~\ref{fig:boolean} show the prompt templates for extracting numeric and boolean inconsistency-related information, respectively.
For generating numeric values like rewards or fee rates, the prompt directly instructs the LLM to `extract numeric values from the provided DApp description'. However, when generating boolean values, which are not explicitly stated in the description, the prompt does more than just instruct the LLM to `answer with yes or no.' It also utilizes CoT (Chain of Thought) patterns to construct $UP_{CoT}$, which guide the LLM in deducing the answer by providing key phrase explanations (e.g., DApp pause, the storage way of NFTs) and illustrative examples. This approach helps the LLM interpret and infer boolean values from the context.
% For example, to extract the reward rate, we set $UP_{it}$ as \textit{``extract numerical information related to the reward from the provided text''}. 
% LLaMA2 shows limitations in answering boolean-type questions in our experiments. To tackle this, we incorporate $UP_{CoT}$, enhancing deductive reasoning with background information and examples. For instance, determining a DApp's pause functionality by answering true or false involves first defining the DApp pause, followed by a step-by-step deductive example.
The complete prompt template for DApp description analysis is formalized as $\{P=\{SP:R+GI\}+\{UP:UP_{it}+UP_{CoT}\}+D\}$, where $D$ represents the raw text of the DApp description. 
% Details on prompt design and refinement are available in our open repository.

\vspace{-0.2cm}
\begin{figure}[hbtp]
    \setlength{\abovecaptionskip}{-0.4cm}
    \setlength{\belowcaptionskip}{-0.6cm}
    \centering
    \includegraphics[width=\linewidth]{./images/boolean2.png}
    \caption{Prompt Template of Boolean Inconsistency-related Information.} \label{fig:boolean}
\end{figure}
\vspace{-0.2cm}

% LLMs rely on a prompt-based learning approach~\cite{prompt}, and the effectiveness of prompt design can significantly affect the performance of the LLM~\cite{chen2023chatgpt}.
% We base our template on LLaMA2's recommended structure~\cite{llama2prompt}, which includes a system prompt ($SP$) and a user prompt ($UP$), symbolized as ${P=SP+UP}$. 

% For the model's role $R$, we define it as an \textbf{expert in blockchain and smart contracts}, aligning with the seven inconsistencies we aim to detect.
% We also incorporate general instructions ($GI$) into the $SP$ for clarity and accuracy, such as \textit{please do not share false information}.
% Our approach to user prompt $UP_{fp}$ design involves categorizing the inconsistencies into groups based on the desired information type, i.e., numeric and boolean information.
% For example, we expect to extract numeric information, e.g., \textit{\{reward:3\%\}} from the description shown in Figure~\ref{fig:reward}.
% The following are examples of our user prompts ($UP_{fp}$).

% \begin{tcolorbox}
% \textbf{Numeric}: Extract numerical information related to the \texttt{\{attribute\}} from the provided text.

% \textbf{Boolean}: \texttt{\{problem\}} + You need to answer `yes' or `no' and provide a concise explanation.
% \end{tcolorbox}

% We notice that LLaMA2 performs poorly when answering our boolean-type questions in our experiment.
% Unlike numeric extraction inconsistency, which typically contains straightforward numbers, boolean-type questions often necessitate interpreting the text and deducing conclusions.
% To address this, we used the chain of thought~\cite{wei2023chainofthought} (CoT) prompt ($UP_{CoT}$), which could guide the LLM step by step with an enriched background to improve the precision of the LLM output. 
% Specifically, we provide basic background information, e.g., the definition of DApp pause, and provide a sample that exemplifies the deduction procedure to show how to infer the result from the given text, e.g., in which case a DApp can be paused inferred from a description.
% Finally, our designed prompt template for DApp description understanding can be represented formally by $\{P=\{SP:R+GI\}+\{UP:UP_{fp}+UP_{CoT}\}\}$.
% All the designed prompts and experiments on how we refine our prompts are detailed in our open repository.

\para{Prompt Segmentation}
%LLMs have a token limit, referring to the maximum number of tokens that the model can process in a single prompt. For LLaMA2, the token limit is 4096~\cite{touvron2023llama}.
The maximum number of tokens that LLaMA2 can process in a single prompt is 4096~\cite{touvron2023llama}.
However, the token length of some DApp descriptions in our dataset exceeds this limit, which yields incorrect answers and unwanted output.
% Therefore, our initial approach involves segmenting the lengthy input into several parts. For this segmentation, we first employed LLaMA2. However, LLaMA2 proved inadequate for this task, as it not only lost significant portions of the original text, but also introduced excessive and redundant information between segments, thereby failing to facilitate effective long-text segmentation.
% As a consequence, we manually set a token limit for each prompt to decrease the number of tokens input into the LLM. We conducted a token length selection experiment with token limit settings of 500, 1000, 1500, 2000, 3000, and 4000 for each input, respectively. The experiment shows that the token length of 3000 has the best performance (see Section~\ref{sec:rq3}); we then divide every DApp description into several groups, ensuring that the token length of each group is less than 3000.
% While this segmentation might sometimes lead to incomplete sentences at the end of an input, large language models, trained on diverse datasets, are adept at understanding context. This enables them to infer meaning and remain coherent even with fragmented input, ensuring that their overall comprehension and performance remain largely unaffected.
% The results show that our token-splitting strategy effectively solve the long-token problem (details are shown in our open repository).
To address this issue, we segment the raw text of the DApp description $D$ by setting a token limit. Every segmentation $D_i$ is further concatenated with the design prompt $SP$ and $UP$ to construct the prompt $P_i$. Through experimentation, we find that a limit of 3000 tokens per segmentation yields the best results (compared to 500, 1000, 1500, 2000, and 4000). This choice effectively handles lengthy descriptions without significantly impacting LLM's comprehension abilities. Although segmentation can result in incomplete sentences, LLMs are skilled in contextual understanding, which allows them to interpret meaning and maintain coherence with fragmented input, preserving their overall comprehension and effectiveness.

\para{Instruction-Tuning}
To enhance LLaMA2's effectiveness for our specific task, we further instruction-tune the model using labeled data on 63 DApp inconsistencies~\cite{icse24-llm}. Specifically, we first segment the raw text of the DApp descriptions, adhering to the 3000 tokens per segmentation, and then construct the LLaMA2 instruction according to our designed prompts $P$ for every segmentation. However, this step yields some wrong responses and useless information, e.g., multiple lines of empty spaces without any text. To refine LLaMA2's responses, we remove redundant words while only retaining outputs that contain the relevant information, and correct any inaccuracies. The revised responses form the basis of our training dataset, which aligns with the structure of the \textit{alpha} dataset, as defined by the LLaMA2 official fine-tuning project~\cite{llamarecipe}. The format can be represented by the tuple (\textit{instruction}, \textit{input}, \textit{output}), where \textit{instruction} refers to the user prompt $UP$, \textit{input} represents DApp description raw text $D$, and \textit{output} denotes the adjusted LLaMA2 response.
After that, we adopt LORA~\cite{hu2021lora}, a famous PEFT (Parameter-Efficient Fine-Tuning)~\cite{peft} method, to train the learnable parameters for our inconsistency information extraction task based on our training dataset.
% To improve LLaMA2's performance on our specific task, we conduct further fine-tuning of the model on the labeled data of DApp inconsistencies~\cite{devlin2018bert,icse24-llm}.
% We collect and label descriptions from 63 DApps, adjusting the LLaMA2's output to align with the labeled results.
% Specifically, we first feed these 63 DApp descriptions to LLaMA2 (conforming to the 3000 token limit and designed prompts) and rectify the output according to the labeled result. 
% We trim the redundant words of LLaMA2 answers while keeping those sentences containing the expected results. We do not directly use the key-value format result as the expected output because we find it significantly undermine the LLM's performance.
% For those correct answers, we trimmed the redundant words while keeping the sentence with the expected results.
% For those wrongly answered questions, we keep our labeled results as the expected output.
The above process achieves an 84\% precision on our test dataset comprising \DAppGT~labeled DApp descriptions (Section~\ref{sec:opencardsoring}), and we finally obtain our model \textsc{HyperText}.
Due to page limitation, we provide a detailed fine-tuning process in our open repository.

% \vspace{-0.2cm}
\subsubsection{Inconsistency-related Attributes Extraction}\label{sec:nltk}
% Considering the speed and accuracy of our DApp description analysis, we do not use LLM to directly obtain concise key-value attributes, which tends to significantly reduce accuracy and efficiency according to our experimental results.
% To address this issue, we adopt NLTK to extract inconsistency-related attributes from the LLM responses.
% Specifically, we first tokenize the response and use the synonym library to help us find the keyword of specific inconsistency~\cite{yu2018ppchecker}. Then, we utilize the token tag information obtained from the part-of-speech (POS) tagging process to interpret and process the text for specific information. For example, to extract \textit{\{reward:3\%\}} from LLM output \textit{``Daily Reward: 3\% of the BNB amount''}, we first locate the keyword \textit{reward}, then check if the following tags exist cardinal number (CD) and find whether a percent sign \% follows this number. Due to the page limit, we show our specific extraction method using NLTK in our open repository.
The output generated by \textsc{HyperText} comprises several sentences assessing the presence of inconsistency-related information within the DApp descriptions. However, these outputs vary in format, necessitating the extraction of uniformly formatted key-value attributes for further comparison with the contract semantics. 

In our experiments, we find that directly extracting key-value attributes using LLM is inefficient and often inaccurate. %For example, our model cannot correctly give answers with instructions that require output in strictly key-value format.
To address this challenge, we employ the NLTK to extract inconsistency-related information from LLM answers and unify them into the key-value format attributes.
For instance, (1) to find the reward rate from HyperText's answer, we first tokenize the sentences and use POS tagging to label the words. Then, we scan for keywords like "reward" and its synonyms extended by NLTK WordNet. The final result is located around the keyword, and we obtain the numeric value based on the digit word tag and symbol `\%'.
(2) It is straightforward to extract the `yes' or `no' boolean symbols from HypetText's answers, as shown in the template (Figure~\ref{fig:boolean}). We directly extract the boolean value from the LLM response.
% Our process involves tokenizing the response, utilizing a synonym library for keyword identification, and applying part-of-speech (POS) tagging for contextual interpretation. 
% For instance, to extract \textit{{reward:3\%}} from an \textsc{HyperText} response \textit{``Daily Reward: 3\% of the BNB amount''}, we first locate the keyword \textit{reward}, then identify any following number and check for a subsequent \%.
% Figure~\ref{fig:nltk} shows the workflow of our \textsc{HyperText} combined with NLTK. The DApp HTML file is first parse to raw text; after concacted with our designed prompts, the instruction will be fed to our HyperText. Then, the NLTK is adopted to extract inconsistency-related attributes, which are used for the inconsistency detection.




\vspace{-0.1cm}
\subsection{Contract Semantic Analysis}\label{sec:sca}
This subsection details how \textsc{HyperCode} recovers high-level semantic features related to inconsistencies from low-level bytecode.
The analysis can be divided into three parts, i.e., decompilation and dataflow analysis, graph analysis, and IR-based symbolic execution.

% First, \textsc{Hyperion} decompiles the contract bytecode and performs dataflow analysis to recover some critical semantics; then, it constructs two graphs to deduce fund transfer information and dependency relationships between state variables. 
% Next, a targeted symbolic execution based on the IR is adopted to check the run-time formal states and obtain information that cannot be determined through static dataflow analysis, e.g., the reward or fee calculation formula. After that, we can obtain the contract semantics for the detection of inconsistencies.

\subsubsection{Decompilation and Dataflow Analysis}\label{sec:decompile}
For contract bytecode analysis, we utilize Elipmoc for decompilation. Elipmoc converts EVM bytecode into a high-level IR, structured in static single assignment (SSA) form, and delineates function borders. Utilizing this IR, we perform dataflow analysis with datalog~\cite{ceri1989you} rules to extract essential semantics for subsequent graph analysis and symbolic execution. This includes defining core IRs related to storage, external calls, and data flow.
% To analyze the contract bytecode, we first adopt Elipmoc to decompile the bytecode.
% Elipmoc can recover the EVM bytecode into a high-level IR. It can also identify the function border according to the decompiled IR, which is in the static single assignment (SSA) form.
% Based on this IR, we perform a dataflow analysis using datalog rules to extract critical information, which we will use in our graph analysis and symbolic execution.
% The core IR instructions related to storage, external calls, and data flow are defined as follows:

\noindent Instruction :- $SSTORE(s,y,z)$ \ | \ $x := SLOAD(s,y)$

\qquad \quad \quad | \ $CALL(s,arg)$ \ 

\qquad \quad \quad | \ $x := CALLPRIVATE(pf,arg)$ \

\qquad \quad \quad | \ $RETURNPRIVATE(t,v)$ \ 

\qquad \quad \quad | \ $x := PHI(y,z)$

Letters ($x$,$y$,$z$,$t$,$v$) denote the variables declared in the IR. The variables $pf$ and $arg$ represent the private function and call arguments, respectively, and $s$ denotes the SSA statement in which an instruction lies.
The semantics of the first three instructions are the same as those of the EVM opcodes. The storage write instruction $SSTORE(s,y,z)$ signifies that the statement $s$ writes variable $z$ to the storage address $y$. And $x:=SLOAD(s,y$) represents the variable $x$ loaded from the storage address $y$ in statement $s$.
Instruction $CALL(s, arg)$ denotes the statement $s$ executes the external contract invocation with arguments $arg$.

The final three instructions - unique to Elipmoc IR - pertain to dataflow and control flow within the IR.
Instructions $CALLPRIVATE$ and $RETURNPRIVATE$ are involved in private function calls:
\textit{x := CALLPRIVATE(pf,arg)} calls the private function $pf$ with arguments $arg$, and $x$ captures the return value. The \textit{RETURNPRIVATE(t,v)} instruction facilitates returning variables $v$ to the caller at target $t$. Lastly, the \textit{x := PHI(y,z)} instruction indicates the flow of variables $y$ and $z$ to $x$, playing a pivotal role in dataflow within the IR.

\begin{table*}[htbp]
\setlength{\abovecaptionskip}{0.cm}
\centering
\caption{Contract IR-level Semantic Relations}\label{tab:relation}
\scalebox{0.88}{
\begin{tabular}{lll}
\toprule
Relation& Notation& Description\\
\midrule
$Constant$& $C(x)=v$& Variable $x$ is inferred to denote a constant value $v$\\
$External call$& $EC(cs, addr, fs)$& Call the function $fs$ of the contract $addr$ at the call site $cs$\\
$Controls$& $Controls(x, s)$& Variable $x$ determines whether the statement $s$ will be executed\\
$MathOp$& $x=Math(op,y,z)$& Variable $y$ and $z$ are two elements of the math operation $op$\\
$CallArg$& $CA(cs,x,i)$& Variable $x$ is the $i$th parameter of the external call whose call site is $cs$\\
$FuncArg$& $FA(fs,x)$& Variable $x$ is the argument of the function whose signature is $fs$\\
$DataFlow$& $\downarrow DF(x,y)$& The value of the variable $x$ will flow to the variable $y$\\
$StatementFunc$& $SF(x,y)$& The statement $x$ is in the public function $y$\\
\midrule
$Transfer$& $Transf(cs, r, a, cf)$& 
\begin{tabular}[l]{@{}l@{}}The variables $r$ and $a$ are the recipient and the transfer amount of call site $cs$\\ respectively in the function whose signature is $cf$\end{tabular}\\
$SenderGuard$& $SG(x, cf)$& 
\begin{tabular}[l]{@{}l@{}}The variable loaded from storage slot $x$ is inferred to be compared with\\ $CALLER$ in function whose signature is $cf$\end{tabular}\\
$StorageInfer$& $ST_{var}(x, cf)$& Variable $var$ is inferred to be stored in slot $x$ in function with signature $cf$
\\
\bottomrule
\end{tabular}}
\vspace{-0.3cm}
\end{table*}

Based on the instruction semantics above, we summarize the high-level semantics in Table~\ref{tab:relation} that we adopt to formulate our dataflow and semantic recovery rules.
The first eight relations in the table are supported by Elipmoc, while the remaining three rules are induced on the basis of the eight relations, which recover a higher-level semantic of contracts.
According to the definition of the seven DApp inconsistencies, there are three of them related to transfer funds (\textit{UR}, \textit{HF}, \textit{UFF}), while the other four are about reading and writing storage (\textit{AL}, \textit{UTS}, \textit{CDS}, and \textit{VNA}).
Therefore, our analysis primarily revolves around two types of operations: \textit{fund transfer} and \textit{specific storage access} (store and load), crucial for pinpointing inconsistencies in contract bytecode.
% Therefore, the \textbf{fund transfer} operations and \textbf{specific storage access operations}  (store and load) are the two main pieces of information when identifying inconsistencies in contract bytecode.

The first induced relationship is \textit{Transfer},
\textit{Transfer} operations are extracted by identifying call operations in the contract bytecode.
From the collected dataset for finding inconsistencies, there are two types of transfers, i.e., Ether and ERC20 token transfer.
ERC20 token transfers are identified through the function signatures mandated by the ERC20 standard: \textit{transfer()} and \textit{transferFrom()}, with respective function signatures 0xa9059cbb and 0x23b872dd~\cite{defitainter}.
In contrast, Ether transfers are characterized by those \textit{CALL} operations, which uniquely do not utilize memory arguments for the call target and transfer amount, referring to the \textit{CALL} instruction semantics~\cite{nftdefects}.
% We find the call to transfer ERC tokens according to the function signatures of those functions mandated by the ERC token standard, i.e., \textit{transfer()} and \textit{transferFrom()}. These two functions are used when transferring tokens through contracts, and their function signatures are 0xa9059cbb and 0x23b872dd, respectively.
% For ether transfer, the \textit{CALL} instruction does not use memory arguments as their call target and transfer amount, which are the third and fourth parameters according to the semantics of \textit{CALL}.
\textsc{HyperCode} identifies these transfer operations and uses rules~\ref{eq:transfer1} to~\ref{eq:transfer3} to determine the critical call sites in the IR.

\vspace{-0.3cm}
\small
\begin{equation}
  \frac{\frac{CA(cs, r, 0)}{CA(cs, a, 1)} \enspace EC(cs, *, fs) \enspace C(fs)="0xa9059..." \enspace SF(cs, cf)}{Transf(cs, r, a, cf)} \label{eq:transfer1}
\end{equation}
\vspace{-0.1cm}
\begin{equation}
  \frac{\frac{CA(cs, r, 1)}{CA(cs, a, 2)} \enspace EC(cs, *, fs) \enspace C(fs)="0x23b87..." \enspace SF(cs, cf) }{Transf(cs, r, a, cf)} \label{eq:transfer2}
\end{equation}
\vspace{-0.1cm}
\begin{equation}
  \frac{!CA(cs, *, *) \enspace CALL(cs, *, r, a, *, *, *, *) \enspace SF(cs, cf)}{Transf(cs, r, a, cf)} \label{eq:transfer3}
\end{equation}
\normalsize

The second induced relationship is \textit{SenderGuard}, which helps us analyze whether some operations are restricted to specific users, e.g., check whether the function caller is the owner.
This relationship is induced by the following rule~\ref{eq:sg}. 
% The statement $s$ loads the variable $x$ from the storage slot $y$, and $x$ is compared with the caller of the function. We can infer that in the function $cf$, there is a sender check that the load variable from storage $y$, which helps us to find the privileged users.
When a statement $s$ retrieves variable $x$ from storage slot $y$ and subsequently compares $x$ with the function's caller, we can deduce that function $cf$ incorporates a sender verification mechanism. This process helps us to identify privileged users within the contract.

\small
\begin{equation}
   \frac{x=SLOAD(s,y) \enspace SF(s, cf) \enspace Comp(x, CALLER)}{SG(y, cf)} \label{eq:sg}
\end{equation}
\normalsize

The other key induction \textit{StorageInfer} is to recover semantics about storage inference.
Our approach involves deducing five distinct types of storage variables from the IR by identifying characteristic features of storage operations. These types include: owner, time, supply, pause, and token URI. Recognizing these variables is essential for pinpointing operations that interact with inconsistency-related variables.
% Specifically, we infer five types of storage variables from the IR by identifying storage operation features, i.e., owner, time, supply, pause, and token uri, which are essential in identifying operations on inconsistency-related variables.
% We identify the storage slots of these variables by combining the function signature identification and pattern matching.
For example, to determine the storage slot for the \textit{owner} variable that represents the contract owner or privileged users, we utilize rule~\ref{eq:owner}.
% For contracts that implement the function $F$ \textit{owner()}, which has a specific signature $SHA3(F)$, we directly infer that the return variable loaded from the slot $y$ can represent the variable ``owner''. In other cases, we refer to the induced pattern $SG$. A comparison of the variable loaded from slot $y$ with the $CALLER$ should be required to be inferred that the variable \textit{owner} is stored in slot $y$.
If a contract implements the function $F$-\textit{owner()} with a specific signature $SHA3(F)$, we infer that the return variable loaded from slot $y$ is indicative of the \textit{owner} variable. In scenarios where \textit{owner()} is not explicitly defined, we resort to pattern matching based on the \textit{SenderGuard} (SG) induction. Specifically, a variable loaded from slot $y$ and compared with the $CALLER$ indicates the \textit{owner} variable is stored in slot $y$.

\vspace{-0.3cm}
\small
\begin{equation}
   \frac{\frac{x=SLOAD(s,y)}{SF(s, cf)} \enspace [C(fs)=SHA3(F) || 
   \frac{Controls(x,*)}{SG(y, cf)}]}{ST_{owner}(y,cf)} \label{eq:owner}
\end{equation}
\normalsize

In our approach, the identification of function signatures is a critical step. We refer to standard interfaces defined in Ethereum Improvement Proposals~\cite{eip} (EIPs) and utilize widely recognized third-party libraries, such as OpenZeppelin~\cite{oz}. This technique allows us to quickly locate critical variables in the contract's bytecode, which is also adopted by other works~\cite{defitainter}. We use this method to find the storage of variables that represent the token supply (e.g., \textit{totalSupply()}), the DApp pause status (e.g., \textit{pause()}), and the token uri (e.g., \textit{tokenURI()}) of the NFT from contract bytecode as shown in rule~\ref{eq:fs}.
For contracts lacking these standard function implementations, our strategy involves a detailed analysis of operational sequences and constraints in the bytecode. We have crafted specific patterns based on source code level features, derived from our ground truth dataset for defining inconsistencies. These patterns facilitate the identification of storage locations by extracting unique features and constraints within the bytecode.

The rules from~\ref{eq:time} to~\ref{eq:pause} outline our variable semantic recovery patterns.
% For the identification of the function signature, we refer to the standard interface declared in the EIP and the widely used third-party library like OpenZepplin. Using the identification of the function signature can help us quickly determine where the critical variable is stored. We use this method to find the storage of variables that represent the token supply, the DApp pause status, and the token uri of the NFT from contract bytecode as shown in rule~\ref{eq:fs}.
% For contracts that do not implement these standard functions, our approach involves analyzing the bytecode's operational sequences and associated constraints. Specifically, we design patterns based on source code level features derived from our ground truth dataset. These patterns enable us to identify storage locations by interpreting the unique characteristics and constraints within the bytecode, even in the absence of standard function implementations.
% Rules~\ref{eq:time} to ~\ref{eq:tokenuri} are variable semantic recovery patterns. 
For example, rule~\ref{eq:time} is employed to identify the state variable storing the DApp's liquidity lock duration.
We ascertain whether the arguments of a public function $x$, combined with the current timestamp (derived from \textit{TIMESTAMP}), flow to a variable $z$, stored in slot $y$. Represented semantically as \verb|lock=now+x|, where $x$ is user-defined lock time, and $now$ is the current timestamp, slot $y$ is inferred to store the lock time.
% We find whether the arguments of the public function $x$, and the current timestamp (obtained by \textit{TIMESTAMP}) can flow to the variable $z$, which is stored in the slot $y$. This semantic can be represented by the \verb|lock=now+x|, while $x$ is the lock time set by the users and now is the current timestamp, the storage slot y is inferred to represent variable lock time.
Likewise, we look for the \textit{ADD} operations (rule~\ref{eq:supply}) and the control semantics (rule~\ref{eq:pause}) to infer the storage of the token supply and the pause variable, respectively. Due to the page limit, please refer to our repository for more details.
% To infer the storage of the token supply variable, we look for \textit{ADD} operations on the token supply as shown in rule~\ref{eq:supply}. If a state variable is retrieved from slot $y$ and subsequently updated after a math addition operation, slot $y$ is inferred to represent the token supply. This is particularly relevant for contracts that do not implement a standard \textit{totalSupply()} interface, where the supply is typically incremented during token minting functions.
% The storage of the \textit{pause} variable is deduced from control semantics.
% As shown in rule~\ref{eq:pause}, when the DApp's pause operation is executed, the stored value in slot $y$ is checked to determine if the DApp is paused. If the loaded variable from slot $y$ influences the setting of the pause status to \textit{True}, we infer that slot $y$ stores the DApp's pause status.
% When operating on pause, its stored value should be checked (whether the DApp has been paused), therefore, if the loaded variable from slot $y$ controls the setting of the variable (\textit{SSTORE}), and the pause status is set to be \textit{True}, the slot $y$ is inferred to store the DApp pause status.

\vspace{-0.2cm}
\small
\begin{equation}
   \frac{x=SLOAD(s,y) \enspace SF(s, cf) \enspace C(fs)=SHA3(F)}{ST_{x}(y,cf) \enspace x\in [supply, pause, token\_uri]} \label{eq:fs}
\end{equation}
\vspace{-0.1cm}
\begin{equation}
   \frac{SSTORE(s,y,z) \enspace \frac{TIMESTAMP(t)}{\downarrow DF(t,z)}  \enspace \frac{FA(fs,x)}{\downarrow DF(x,z)} \enspace SF(s,cf)}{ST_{time}(y,cf)} \label{eq:time}
\end{equation}
\vspace{-0.1cm}
\begin{equation}
   \frac{x=SLOAD(s,y) \enspace r = MathOp(+,x, *) \enspace 
\frac{SSTORE(a,y,R)}{\downarrow DF(r,R)}}{ST_{supply}(y,cf)} \label{eq:supply}
\end{equation}
\vspace{-0.1cm}
\begin{equation}
   \frac{x=SLOAD(s,y) \enspace SF(s, cf) \enspace \frac{Controls(x,a)}{SSTORE(a,y,T)} \enspace C(T)=True}{ST_{pause}(y,cf)} \label{eq:pause}
\end{equation}
\normalsize
% \begin{equation}
%    \frac{x=SLOAD(s,y) \enspace SF(s, cf) \enspace C(fs)=SHA3(F)}{ST_{token\_uri}(y,cf)} \label{eq:tokenuri}
% \end{equation}

\subsubsection{Graph Analysis}
After we recover the high-level semantics of the IR of the contract, we construct a graph to obtain the connection between the critical information that we extracted in the contract.
This graph contains two subgraphs, i.e., the fund transfer graph (FTG) and the state variable dependency graph (SDG). These subgraphs facilitate our analysis of contract semantics, particularly in relation to inconsistency attributes.
% There are 3 kinds of nodes and 3 kinds of edges in this graph.

The graph construction is grounded on three key relations: \textit{Transfer}, \textit{SenderGuard}, and \textit{StorageInfer}. The $Transfer(cs,r,a,cf)$ relation is utilized to identify recipient nodes and the corresponding transfer amount edges for each transfer operation. We also identify whether the transfer amount to some nodes is part of the amount transferred to users to identify receiving fee operations, and whether there exists a recipient who can withdraw the contract balance.

% Specifically, we utilize the relations \textit{Transfer}, \textit{SenderGuard}, and \textit{StorageInfer} to build the graph. Relation $Transfer(cs,r,a,cf)$ identifies recipient nodes (e.g., nodes R1, R2, and R3 in Figure~\ref{fig:graph}), and the transfer edge (e.g., directed edges a1, a2, and a3) of each transfer operation.
% We also identify whether the transfer amount to some nodes is part of the amount transferred to users (e.g., a3 is included in a1) to identify receiving fee operations.

For state variable dependencies, we start by identifying state variable nodes (e.g., $ST_x$) using $ST_{var}(x,cf)$. 
Then, through the \textit{SenderGuard} relationship, we determine state variables that are conditionally manipulated based on sender verification (e.g., pause status $ST_{pause}$ is controlled by the owner). This step is crucial for mapping the complex dependencies of state variables within the contract and finding those privileged operations.

% Then, according to the dependency relationship \textit{SenderGuard}, we infer the state variables that operate in the context with the sender check.
In our graph analysis, we delve into the roles of recipients and their associated high-level features. Additionally, we organize the extracted information at the function level to guide our subsequent symbolic execution. Two essential features are extracted for this purpose: $\overrightarrow{FTG}(cs,r,a,cf,p)$ and $\overrightarrow{SDG}(cs,x,cf,d)$, where $p$ denotes the inferred privileged owner, e.g., who can withdraw the contract balance, and $d$ represents the dependency relationships among state variables.

% Furthermore, to guide our following symbolic execution, we group the information into function-level. Two features are extracted, i.e.,
% $\overrightarrow{FTG}(cs,r,a,cf,p)$ and $\overrightarrow{SDG}(cs,x,cf,d)$, while p is the inferred owner (or privileged user), e.g., who can withdraw all the contract balance, and d is the dependency relationship of state variables.

% \vspace{-0.3cm}
% \begin{figure}[!htbp]
%     \setlength{\abovecaptionskip}{-0.1cm}
%     \centering
%     \includegraphics[width=3in]{./images/graph_analysis.jpg}
%     \caption{Graph analysis of our approach.} \label{fig:graph}
% \end{figure}
% \vspace{-0.2cm}

\subsubsection{IR-based Symbolic Execution}
% After we extracted the basic features, a symbolic execution framework is adopted to help obtain the runtime states and validate the critical attributes.
% There are two motivations for why we design a symbolic execution framework on the IR from scratch.
With the extraction of basic features completed, we proceed with an IR-based symbolic execution framework to obtain runtime states and validate critical attributes. %This framework is designed from scratch for two primary reasons:
% First, the IR constructs a complete control flow graph, while the traditional symbolic execution should run as a complete execution to resolve all jump targets of basic blocks~\cite{grech2022elipmoc}. This enables us to reduce the scope of the execution as we just need to execute the critical functions and paths.
%First, unlike traditional symbolic execution that necessitates complete execution to resolve all jump targets of basic blocks~\cite{luu2016making,chen2021defectchecker}, our IR-based approach takes advantage of a fully constructed control flow graph~\cite{grech2022elipmoc}. This allows for a more focused execution, limiting the scope to only critical functions and paths, thus enhancing efficiency.
% Second, we can apply the information from the dataflow analysis and recovered semantics to help us determine which statement in the IR needs to be checked and which variables are used in this program point. In other words, the semantics recovered from the IR can be used directly in the symbolic execution based on the IR.
%Second, the IR-derived semantics directly inform the symbolic execution process. The dataflow analysis and recovered semantics guide us in determining which statements in the IR require checking and which variables are used or defined at given program points. Therefore, the symbolic execution on this IR can perfectly integrate with the dataflow analysis results.
The IR, distinct from EVM opcodes, features unique instructions (as detailed in section~\ref{sec:decompile}). 
% For instance, the traditional \textit{PUSH} opcode is supplanted by \textit{CONST} in IR. A key aspect of IR is its delineation of function borders, effectively segregating basic blocks into public and private functions. Public functions are identified by their signatures in the bytecode, while private functions are extracted from repeatedly called basic block groups. 
The interaction between identified public and extracted private functions is managed by \textit{CALLPRIVATE} and \textit{RETURNPRIVATE} instructions, which facilitate parameter and result passing in IR CFG.
% Different from the EVM opcode, the IR has its own instructions, as illustrated in the section~\ref{sec:decompile}.
% For example, the \textit{PUSH} opcode is replaced by the instruction \textit{CONST}, and there is no stack or memory usage, which is more like the source code.
% The main feature of the IR is to recover function borders that divide basic blocks into specific functions. There are two types of function in the IR, public function and private function. The public function is named by the function signature identified in the contract bytecode.
% If a group of basic blocks is called multiple times to implement some functions, they can be extracted to a private function, which can be called by public functions.
% Instructions \textit{CALLPRIVATE} and \textit{RETURNPRIVATE} are introduced to manage the call flow between public functions and private functions, which pass the parameters and calculation results of private functions.
% An exemplary IR private function call is depicted in Figure~\ref{fig:ir}. Specifically, a public function $PF$ invokes the private function $F1$ with arguments $vargs$. Within $F1$, the return variable $R2$ of another private function $F2$ operates on $vargs_{f2}$. The execution bifurcates at the \textit{JUMPI} instruction based on the condition $cond$. If $cond$ is true, block \textit{TB} executes, and variable $X$ flows to the return variable $R1$ via the \textit{PHI} instruction. Conversely, if $cond$ is false, block \textit{FB} executes, returning a constant value 0x0 to $PF$. 
The \textit{PHI} instruction is critical in merging variables from divergent control flows. The first element indicates the in-loop variable that determines the loop exit condition, while the second acts as an out-loop bound checker.
% For instance, if $cond$ is false, $X$ becomes undefined, and $Y$ (0x0) is used instead. 
% In loop scenarios, the first \textit{PHI} element indicates the in-loop variable, crucial for determining loop exit conditions, while the second element acts as an out-loop bound checker.
Due to page limitation, we show an exemplary IR CFG in our repository.
% To address the issue of variable definition across different symbolic execution paths, we establish a separate storage space for private function variables. This ensures that once the control flow exits a private function, the previously defined variables are cleared, preventing the reuse of outdated states in subsequent function calls.

% Figure~\ref{fig:ir} shows an example of the private function call feature of the contract IR.
% The public function $PF$ calls the private function $F1$ with arguments $vargs$.
% In $F1$, $R2$ is the return variable of the private function $F2$, which operates on $vargs\_f2$.
% Then, the \textit{JUMPI} instruction divides the execution into two branches. If $cond$ is true, the block \textit{TB} will be executed, and the variable $X$ will flow to the return variable $R1$ by instruction $PHI$. Instead, if $cond$ is false, the variable $Y$, which is a constant value 0x0 in block \textit{FB} will return to $PF$.
% The \textit{PHI} instruction is special in IR. The two elements used by \textit{PHI} $X$ and $Y$ are variables in different control flows. For example, the variable $X$ is declared in block \textit{TB}, but if $cond$ is false, the variable $X$ is an undefined variable. In this case, the variable $Y$ with the value 0x0 is used to return from the private function. According to the design of this IR, \textit{PHI} exists whether there is a loop, the first element, e.g., $X$ is the in-loop variable, which can determine the jump-out condition, while $X$ represents the out-loop variable that serves as a bound checker.
% Furthermore, to bypass the bi-usage of defined variables in different symbolic execution paths, we create an individual space for private function variables storage. When the control flow jumps out of the private function, the cached defined variables will be cleared to make sure that the next private function call will not use the former cached states.

% \vspace{-0.1cm}
% \begin{figure}[!htbp]
%     \setlength{\abovecaptionskip}{-0.4cm}
%     \centering
%     \includegraphics[width=\linewidth]{./images/ir_se_2.jpg}
%     \caption{Features of our IR CFG.} \label{fig:ir}
% \end{figure}
% \vspace{-0.3cm}

Based on the IR CFG illustrated above, \textsc{Hyperion} builds an extensible symbolic execution framework from scratch that makes use of the completeness of IR CFG while incorporating the semantics of each instruction and the dataflow analysis results.
To guide the symbolic execution process, we use dataflow information to monitor critical variables involved in key operations and their flows, e.g., variables flow from and to storage slots (via SSTORE and SLOAD), to formulate induction rules. Graphs extracted based on contract semantics using dataflow analysis and datalog rules label key variables (e.g., transfer amounts) and statements (e.g., external calls) at the function level. They also highlight dependencies among core state variables, e.g., which state can be changed by the contract’s privileged user. These graphs record information identical to the contract IR operated by symbolic execution, guiding which functions to test which variables to load, and at which program point to check the execution states.
This framework can support our testing during symbolic execution and check critical states for contract semantics recovery, which is also extensible for programming more rules.


\vspace{-0.2cm}
\subsection{Inconsistency Detection}
% We use the obtained attributes from DApp descriptions and contract semantics to identify inconsistencies in DApps. 
To detect the inconsistencies, the frontend analysis yields key-value information for critical attributes, e.g., fee rate. The backend analysis maps these attributes to key variables (e.g., transfer recipient and amount, token uri) and operations (e.g., ether/token transfer, contract states modification) that are identified using induction rules and graph analysis during symbolic execution.
Specifically, the attributes extracted by \textsc{HyperText} are denoted as \textit{F}, with each attribute $A_f$ assigned a numeric ($n$) or boolean ($b$) value $V$, based on the inconsistency type. For contract semantics, \textsc{HyperCode} identifies attributes $A_b$ and their values $V$, as well as expressions $F_{expr}$ from symbolic execution ($SE$).
% For each attribute $A_f$, \textsc{Hyperion} ascertains its value $V$, which could be either numeric ($n$) or boolean ($b$), depending on the inconsistency type. Similarly, for the contract's back-end semantic analysis, it identifies corresponding attributes $A_b$ and their values $V$, alongside formal expressions $F_{expr}$ derived from the symbolic execution ($SE$) of the contract IR, which is particularly essential for inconsistencies related to transfer operations such as \textit{Reward}, \textit{Fee}, and \textit{Fund Flow}.

\small
\vspace{-0.2cm}
\noindent\begin{minipage}{.4\linewidth}
    \begin{equation}
      F: \{A_f:V\}, V\in n|b \label{eq:fe}
      \nonumber
    \end{equation}
\end{minipage}%
\begin{minipage}{.6\linewidth}
    \begin{equation}
B: \{A_b:V, F_{expr}\}, \frac{V\in n|b}{F_{expr}\to SE} \label{eq:be}
\nonumber
    \end{equation}
\end{minipage}
\normalsize
% \vspace{-0.2cm}

% It is noticeable that our inconsistency detection involves requesting public nodes through the Web3 API~\cite{web3py}. We use \textit{getCode} to fetch the bytecode of a contract and use \textit{getStorageAt} to obtain storage data in a specific slot and offset from a contract account. Our \textsc{Hyperion} supports inconsistencies detection for DApps on ten mainstream blockchain platforms. The specific inconsistency detection rules for each inconsistency are shown in the following paragraphs.

To facilitate this detection, \textsc{Hyperion} utilizes public nodes via the Web3 API~\cite{web3py}, employing methods like \textit{getCode()} for bytecode retrieval and \textit{getStorageAt()} for accessing specific storage data. In total, our \textsc{Hyperion} supports inconsistency detection across 13 blockchain platforms.

\textit{UR} inconsistency is flagged when the DApp's description cites a fixed reward rate $A_{f(r)}$. Yet, the contract's semantic analysis reveals a transfer amount $F_{expr_{ta}}$ dependent on dynamic factors (like contract balance), with the transfer target $F_{expr_{tt}}$ being the user (\textit{CALLER}). In \textit{HF} inconsistency detection, \textsc{Hyperion} examines DApp descriptions for fee claims and analyzes contract semantics for transfer amounts to specific addresses. An example involves symbolically expressing the transfer amount as \textit{bvudiv\_i(Ia\_store-1-*Iv, 100)}, with \textsc{Hyperion} then querying public nodes for corresponding storage values to calculate and compare fee rates \textit{Ia\_store-1/100} against those mentioned in the DApp description. The modifiable status of fee variables is also reported through SDG.
% The \textit{Reward} inconsistency is identified when the DApp description extracts the reward rate $A_{f(r)}$ as a constant numeric value while the contract semantic analyzer identifies the transfer amount $F_{expr_ta}$ depending on a non-determined environment variable, e.g., contract balance, while the transfer target $F_{expr_tt}$ is the user (denoted by \textit{CALLER} in the contract IR).
% In \textit{Fee} inconsistency detection, \textsc{Hyperion} examines whether there is a fee claim on the DApp description.
% The contract semantics about transfer amount to a determined address (i.e., constant address or address-type state variable) from the formal expression is utilized. For example, when \textsc{Hyperion} identifies the transfer amount expressed symbolically by \textit{bvudiv\_i(Ia\_store-1-*Iv, 100)} ($Iv$ represents the fund transferred from users) to the address \textit{Concat(0, Extract(159, 0, Ia\_store-0-))}, it then requests the remote public node to get the storage value at storage slot 1 of this contract's storage. The fee is calculated using this formula to obtain a fee rate \textit{Ia\_store-1/100}, which will be compared by \textsc{Hyperion} with the fee rate extracted from the DApp description. 
\textit{UFF} inconsistency is identified when the DApp description omits mention of fund withdrawal by specific or privileged users, yet contract semantics suggest otherwise.
% The other inconsistency related to transfer operation, Fund Transfer, is identified when the DApp description does not reveal that the fund can be withdrawn by a specific or privileged user, while the contract semantics are recovered to reveal that the contract balance, or any amount of fund, can be withdrawn by privileged users from our graph analysis.

For \textit{AL} inconsistency, \textsc{Hyperion} assesses both the front-end lock time description and the contract's ability to modify this duration. An inconsistency is noted if the lock time is alterable, irrespective of whether users are informed or not.
% To detect \textit{Liquidity Lock Time} inconsistency, \textsc{Hyperion} checks whether the identified lock time can be modified from contract semantics and judge if there is a lock time description on the DApp front-end. It is noticeable that no matter whether there is a description of lock time, the modifiable state of the lock variable is considered as this inconsistency, as the DApp developer can modify the lock time regardless of users' willingness. 
% Similarly, the description of the token supply from the front-end is extracted, and whether the token supply can be incremented without restriction is inferred from contract semantics; the inconsistency exists when there is a limited token supply but no restriction in the contract semantics and no token supply claimed while contract indeed supporting unrestricted token minting is also considered as an inconsistent behavior.
In \textit{UTS} analysis, \textsc{Hyperion} contrasts the front-end description with the contract's token minting capabilities. 
Two scenarios are flagged as inconsistencies:
(1) when a limited token supply is claimed, but the contract allows unconstrained minting; (2) when the front-end does not explicitly mention any limit on the number of tokens, but the contract is designed to support unconstrained minting.

For the boolean inconsistencies \textit{CDS} and \textit{VNA}, \textsc{Hyperion} extracts the boolean value inferred from the DApp description. The modifiability of the DApp status can be obtained from contract semantics by rule~\ref{eq:pause} when performing symbolic execution, so as to report the \textit{CDS} inconsistency. 
To obtain the storage way of NFTs, we request the public node to obtain the base URI of DApp NFTs (considered as the prefix of stored metadata of NFTs), which is stored in the inferred variable from contract semantics. We judge whether the NFT is stored in decentralized storage services (such as IPFS~\cite{ipfs} and Arweave~\cite{arweave}) or in centralized ways (HTTPS and Base64~\cite{base64}) from this prefix. \textsc{Hyperion} compares this information with the storage way inferred from the description to report \textit{VNA}.


==> icse2025-p517/05_evaluation.tex <==
\vspace{-0.2cm}
\section{Evaluation}
\subsection{Experiment Setup}
The experiment was conducted on a server running Ubuntu 20.04.1 LTS and equipped with 128 Intel(R) Xeon(R) Platinum 8336C @ 2.30GHzE CPUs, and 2 NVIDIA A800 80GB PCIes.

\para{Dataset} We used two datasets to evaluate \textsc{Hyperion}. 
The first one is the ground truth dataset, which contains \DAppGT~DApps we labeled for inconsistency definition in Section~\ref{sec:opencardsoring}. 
The second dataset contains \WildDApp~real-world DApps with their available HTML files, contract addresses, and platforms. Notably, \textsc{Hyperion} is compatible with contracts written in Solidity, regardless of whether they are deployed on Ethereum, e.g., BNB Chain~\cite{bnbsmartchain}, Polygon~\cite{polygon}. We crawled them from the DeFi and NFT categories on DappRadar and DAppBay.
% To our knowledge, this data set is the largest open DApp dataset with DApp websites and smart contracts, covering ten blockchain platforms, which can be useful for future work.
%Both of these two datasets are open source in the open repository.

\para{Evaluation Metrics} We summarize the following research questions (RQs) to evaluate \textsc{Hyperion}.
\begin{enumerate}[RQ1.]
\item How effective is \textsc{Hyperion} in detecting inconsistencies in our ground-truth DApp dataset?
\item How is the performance of \textsc{Hyperion} in detecting inconsistencies in the large-scale DApp dataset?
\item What is the efficacy of \textsc{HyperText} and \textsc{HyperCode} in analyzing DApp descriptions and contract semantics, respectively?
\end{enumerate}

\subsection{Answer to RQ1: Effectiveness in the Ground Truth Dataset}
To answer RQ1, we run \textsc{Hyperion} in our ground truth dataset of \DAppGT~DApps. The detection result is shown in Table~\ref{tab:gt_res}, which outlines the number of each type of inconsistency (Incs) in the dataset, true positives (TP) correctly identified, false negatives (FN) not detected, and false positives (FP) wrongly identified by \textsc{Hyperion}. We use formulas $\frac{\#TP}{\#TP+\#FN}\times 100\%$ and $\frac{\#TP}{\#TP+\#FP}\times 100\%$ to calculate the recall (Rec) and precision (Prec) rate, respectively.
Furthermore, we also calculate the overall precision and recall of \textsc{Hyperion} on the ground truth dataset.
Using overall precision as an example, the overall result can be calculated by the formula $\frac{\sum_{i = 1}^{n}p_{c_i}\times|c_i|}{\sum_{i = 1}^{n}|c_i|}$, in which $p_{c_i}$ represents the precision to detect inconsistencies $i$, and $|c_i|$ is the number of inconsistencies $i$. This method is also adopted by other works~\cite{nftdefects, chen2021defectchecker}.
% The first column shows the DApp inconsistency types, and the second column represents the number of inconsistencies of each type in our ground truth dataset.
% The third and fourth columns show the true positives (TP) reported by \textsc{Hyperion}, and the false negatives (FN) missed by it. We then use $\frac{\#TP}{\#TP+\#FN}\times 100\%$ to calculate the recall rate of \textsc{Hyperion}.

The results show that the overall precision and recall of \textsc{Hyperion} are 92.06\% and \OverallRecall, respectively.
The detailed false negative and false positive analysis is discussed and illustrated in our answer to RQ3 (see Section~\ref{sec:rq3}).

\vspace{-0.3cm}
\begin{table}[!htbp]
\setlength{\abovecaptionskip}{-0.4cm}
    \begin{center}
        \caption{Detection Result in Ground Truth Dataset.}
        \label{tab:gt_res}
        \resizebox{\columnwidth}{!}{
    \centering
    \begin{tabular}{l||l|l|l|l|l|l}
    \hline
        \textbf{DApp Inconsistency} & \# \textbf{Incs} & \# \textbf{TP} & \# \textbf{FN} & \# \textbf{FP} & \textbf{Rec} (\%) & \textbf{Prec} (\%) \\ \hline
        \textit{Unguaranteed Reward} & 19 & 12 & 7 & 0 & 63.2 & 100.0 \\ \hline
        \textit{Hidden Fee} & 21 & 17 & 4 & 0 & 81.0 & 100.0 \\ \hline
        \textit{Adjustable Liquidity} & 4 & 4 & 0 & 0 & 100.0 & 100.0 \\ \hline
        \textit{Unconstrained Token Supply} & 8 & 8 & 0 & 3 & 100.0 & 72.7 \\ \hline
        \textit{Unclaimed Fund Flow} & 12 & 12 & 0 & 2 & 100.0 & 85.7 \\ \hline
        \textit{Changeable DApp Status} & 4 & 4 & 0 & 0 & 100.0 & 100.0 \\ \hline
        \textit{Volatile NFT Accessibility} & 1 & 1 & 0 & 0 & 100.0 & 100.0 \\ \hline
    \end{tabular}
}
    \end{center}
    \vspace{-0.3cm}
\end{table}

\vspace{-0.1cm}
\subsection{Answer to RQ2: Detection in a Large-scale Dataset}
To answer RQ2, we run \textsc{Hyperion} on \WildDApp~unlabeled DApps obtained from DAppRadar and DAppBay. 
The experimental results given in Table~\ref{tab:ls_res} (the second and third columns) show the frequency of each DApp inconsistency in this dataset.

% The result shows that \textsc{Hyperion} reports 245 DApps with at least one inconsistency.

To evaluate the performance of \textsc{Hyperion} in finding inconsistencies in the large-scale dataset, we refer to a random sampling method based on the confidence interval~\cite{confidenceinterval} to generalize the population of the total number of problems found for this inconsistency, which is also adopted in the previous works~\cite{nftdefects}.
Specifically, to establish the sample size of each inconsistency, we set a confidence interval of 10 and a confidence level of 95\% and calculate the number of samples (S, the fourth columns in Table~\ref{tab:ls_res}) that we need to collect~\cite{confidenceintervalcalculator}. 
The calculated results of the seven inconsistencies are 18, 44, 13, 60, 67, 34, and 49, respectively. The evaluation dataset is then randomly sampled according to the result and manually labeled by three authors of this paper.
We analyzed all the reported samples of \textit{UR} and \textit{AL} as the total number reported is close to the calculated number that should be sampled for these two inconsistencies.
% We separated false positives (FP) and true positives (TP) to analyze the performance of \textsc{Hyperion}, which is also adopted by other related works~\cite{nftdefects,luu2016making,kalra2018zeus}.

\vspace{-0.3cm}
\begin{table}[htbp]
\setlength{\abovecaptionskip}{-0.4cm}
    \begin{center}
        \caption{Detection Result in Large-scale Dataset.}
        \label{tab:ls_res}
        \resizebox{\columnwidth}{!}{
    \centering
\begin{tabular}{l||l|l|l|l|l|l}
    \hline
        \textbf{DApp Inconsistency} & \# \textbf{Incs} & \textbf{Per} (\%) & \# \textbf{S} & \# \textbf{TP} & \# \textbf{FP} & \textbf{Prec} (\%) \\ \hline
        \textit{Unguaranteed Reward}             & 22 & 2.63   & 22 & 20 & 2 & 90.9 \\ \hline
        \textit{Hidden Fee}                & 77 & 9.22 & 44 & 38 & 6 & 86.4 \\ \hline
        \textit{Adjustable Liquidity} & 15 & 1.80 & 15 & 15 & 0 & 100.0 \\ \hline
        \textit{Unconstrained Token Supply}       & 159 & 19.04  & 60 & 46 & 14 & 76.7 \\ \hline
        \textit{Unclaimed Fund Flow}          & 223 & 26.71 & 67 & 66 & 1 & 98.5 \\ \hline
        \textit{Changeable DApp Status}        & 51 & 6.12   & 34 & 34 & 0 & 100.0 \\ \hline
        \textit{Volatile NFT Accessibility} & 98 & 11.74   & 49 & 49 & 0 & 100.0 \\ \hline
    \end{tabular}
}
    \end{center}
    \vspace{-0.5cm}
\end{table}
% \vspace{-0.3cm}

The fifth and sixth columns in Table~\ref{tab:ls_res} show precision evaluation on the randomly sampled dataset, divided into TPs (268) and FPs (23) (we manually labeled all DApp with \textit{UR}, and \textit{AL} inconsistencies to make the results more reliable), which is also adopted by other related works~\cite{nftdefects,luu2016making,kalra2018zeus}.
The precision rate of \textsc{Hyperion} in the analysis of each inconsistency is shown in the seventh column.

The results show that for \textit{UR}, \textit{HF}, \textit{UTS}, and \textit{UFF} inconsistencies, \textsc{Hyperion} reports them with a precision of 90.9\%, 86.4\% 76.7\%, and 98.5\%, respectively, and reaches a precision of 100\% when analyzing other types of inconsistency.
% We use the formula $\frac{\sum_{i = 1}^{n}p_{c_i}\times|c_i|}{\sum_{i = 1}^{n}|c_i|}$ to calculate the overall precision of \textsc{Hyperion}, in which $p_{c_i}$ represents the precision to detect inconsistencies $i$, and $|c_i|$ is the number of inconsistencies $i$. This calculation is also adopted by other works~\cite{nftdefects, chen2021defectchecker}.
Our tool \textsc{Hyperion} reaches an overall precision of \OverallPrecision.
%The following section will illustrate the false positive analysis by answering RQ3.
In addition, we have further checked TPs (268 DApps) from the sampled dataset based on Hyperion's reports. We find that 67 (\textbf{25\%}) of them are now \textbf{inaccessible} within just 3 months. Of the remaining accessible DApps, 41 (\textbf{15.3\%}) DApps are labeled as \textit{high risk} by DAppRadar. These numbers underscores the threats these DApps pose to users’ assets.

\vspace{-0.1cm}
\subsection{Answer to RQ3: Evaluation of Respective Performance}\label{sec:rq3}
\vspace{-0.1cm}
% To answer RQ3, we assess two primary components of \textsc{Hyperion}: the DApp description analyzer and the contract semantic analyzer. This evaluation is informed by the incidence of false positives and negatives noted in our preliminary experiments.
% We utilized our ground truth dataset and a randomly sampled subset from the larger dataset for this evaluation.
We observe that \textsc{Hyperion} has some FP and FN in the former two RQs.
However, we do not know whether these inaccuracies are stemmed from \textsc{HyperText} or \textsc{HyperCode}.
Therefore, we propose RQ3, evaluating \textsc{Hyperion}'s two analyzers' performance, respectively.
Our evaluation utilizes the ground truth dataset in RQ1 and the randomly sampled dataset used in RQ2.

\subsubsection{HyperText}
The development of \textsc{HyperText} involved multiple evaluations and experiments mentioned in Section~\ref{sec:llm}. Starting with the design of effective prompts, we progressed through prompt segmentation and instruction-tuning our model.
Due to the page limit, detailed experimental results and related datasets are presented in our open repository.

For the performance evaluation, three authors manually reviewed the DApp descriptions and the corresponding outputs of our \textsc{HyperText}. This involved reading the website pages and verifying the accuracy of extracted attributes. 
In the ground truth dataset, we noted instances where \textsc{HyperText} failed to extract reward or fee information from DApp descriptions, leading to missed inconsistency. The precision and recall of \textsc{HyperText} are 100\% and 92.8\%.
In the large-scale dataset, we find that \textsc{HyperText} exhibited misclassification errors due to the existence of prompt keywords. 
% For instance, in the case of the DApp \textit{Alchemix}, the LLM erroneously related the phrase ``total expected supply after 3 years: 100\%'' to token supply due to the presence of keywords ``total'' and ``supply''. 
For example, in the DApp \textit{Alchemix}~\cite{alchemix}, \textsc{HyperText} mistakenly categorized the text ``total expected supply after 3 years: 100\%'' as token supply information, misled by the keywords `total' and `supply', despite the context indicating a time duration rather than token quantity.
The overall precision of \textsc{HyperText} in the large-scale dataset is 95.9\%.
Additional examples of \textsc{HyperText}'s incorrect responses are available in our repository.


\subsubsection{HyperCode}
To evaluate \textsc{HyperCode}, we compare its output against the contracts code to identify FNs and FPs. The precision and recall of \textsc{HyperCode} in the ground truth dataset are 92.06\% and 84.06\%, respectively, and the precision in the large-scale dataset achieves 92.1\%.

\para{False Negatives}
To analyze false negatives, we refer to the ground-truth dataset used in RQ1.
We find that there are some FNs of \textit{UR} and \textit{HF} inconsistencies due to path explosion in symbolic execution and missing detectable fee transfer operations. 
% We put specific FN samples in our repository.
% (1) \textsc{Hyperion} fails to reach the program checkpoints due to the path explosion during symbolic execution on contract IR. Specifically, some contracts contain a large number of branches in their IR-based CFG, leading to a huge search space.
% As we limited the maximum depth of path searching and loop times to avoid path explosions in \textsc{Hyperion}, some potential checkpoints are not reached by it, which fails to be detected by \textsc{Hyperion}.
% (1) \textsc{HyperCode} struggles with path explosion during symbolic execution on contract IR, leading to missed program checkpoints. This issue arises primarily due to the extensive branches in the IR-based CFG of some complicated contracts, creating a vast search space. Constraints set in \textsc{HyperCode}, such as path search depth and loop iteration limits to avoid the path explosion, contribute to its inability to reach deep checkpoints.
(1) \textsc{HyperCode} sets constraints such as path search depth and loop iteration limits to avoid the path explosion, which contributes to its inability to reach deep checkpoints in the IR CFG of some complicated contracts.
% (2) For \textit{Fee} inconsistency, there are some missing cases because the state variables that store fees are not involved in the transfer operation, which is the key property to detect \textit{Fee} inconsistencies. 
% Although the recorded fee rate is inconsistent with the DApp description (e.g., 10\% sell fee in the DApp description but 25\% implemented in the smart contract), we cannot locate the fee transfer operation to find the inconsistency, which generates false negatives.
(2) In detecting \textit{HF} inconsistencies, \textsc{HyperCode} misses cases where state variables storing fees are not part of the transfer operation. Consequently, even if there is an inconsistency between the DApp description and the actual fee rate stored in the state variable, the absence of a detectable fee transfer operation results in false negatives.

\para{False Positives}
% There are also some false positives in our large-scale experimental results. 
% (1) To detect \textit{Token Supply} inconsistency, the contract semantic analyzer relies on the standard ERC interface \textit{totalSupply()} to identify the storage of the state variable that stores the total token supply. However, some contracts implement this interface in a way that does not return this state variable directly, which is critical in our identification method. 
% For example, they use \verb|_currentIndex-_startTokenId()|~\cite{8liens} or the array length \verb|_allTokens.length|~\cite{MutantCats} to denote total supply, which makes our comparison pattern fail to cover.
% In addition, we find that there is one false positive because the condition check is designed after the add operation on the total supply state variables~\cite{MCHCoin}. As our pattern is to check whether there is a protection comparison with token supply before the supply addition, the false positive is reported.
(1) To identify \textit{UTS} inconsistencies, our \textsc{HyperCode} uses the ERC interface \textit{totalSupply()} to locate the state variable for total token supply. However, some contracts do not directly return this variable when implementing the interface. For instance, contracts using \textit{\_currentIndex-\_startTokenId()}~\cite{8liens} or \textit{\_allTokens.length}~\cite{MutantCats} for total supply deviate from our pattern. Moreover, an FP is noted where the condition check occurs after adding to the total supply state variable~\cite{MCHCoin}, contradicting our pattern of requiring a protective comparison before such an addition.
% (2) As our contract semantics are recovered from bytecode, which misses some source code-level semantics, the contract semantic analyzer considers a split payment to different preset addresses as fee receivers, which can be a normal purchase payment.
% For example, the contract~\cite{feefp} contains a function called \textit{payment()} (lines 201 to 211), which divides the user's payment into two preset accounts \verb|trustedWallet_A| and \verb|trustedWallet_A|. In fact, no additional fee is charged, but two accounts share the user's payment.
(2) \textsc{HyperCode} incorrectly identifies split payments to preset addresses as fee transactions, which could actually be regular payments. For example, a contract's \textit{payment()} function (lines 201 to 211) splits the user's payment between two trusted wallets~\cite{feefp}. In contrast to being a \textit{Hidden Fee}, it is merely a division of a user's payment across two accounts.
(3) For \textit{UFF}, false positives exist when the contract logic actually stipulates transferring all remaining funds when the balance is insufficient for the user's earnings.
(4) When detecting \textit{UR}, \textsc{HyperCode} incorrectly views percentage-based transfers as a profit distribution, while the function's purpose is to manage funds stuck in the contract.
Specific samples are provided in our repository.

Furthermore, the dataflow analysis on the decompiled IR reduces the 88.7\% of functions to be tested on average (in our large-scale experiments) when \textsc{HyperCode} performing IR-based symbolic execution, improving the detection efficiency.

\para{Comparison Experiment} 
We conducted
a survey on works published in top journals/conferences on
SE/Security and found that the proposed inconsistencies have
not been covered before, while NFTGuard~\cite{nftdefects} and Pied-Piper~\cite{piedpiper} have similar detection patterns for contract semantics of UTS and UFF, respectively. We compare \textsc{HyperCode} with NFTGuard, as Piped-Piper is not fully open source (missing the fuzzing part). We randomly select 50 DApps from the large-scale dataset and collect their contract sourcecode (NFTGuard only supports sourcecode). The result shows that \textsc{Hyperion} finds 16 problematic \textit{UTS} contract behaviors with a precision of 75\%, while NFTGuard does not report any bugs. Details are provided in our repository.

% Due to the page limit, our repository shows specific samples of false negatives and positives.

% 一些similar的pattern
%\para{Similar Patterns of other works}
%To find out whether there are contract analysis tools that can detect similar issues in contracts, we first refer to a list of vulnerability detection tools from work~\cite{nftdefects}, and extend this list by surveying new papers that they do not yet cover. Pied-Piper~\cite{piedpiper} is a missed fuzzing tool that can detect \textit{Arbitrary Token Transfer}, similar to our \textit{Fund Flow} Inconsistency pattern. In addition, NFTGuard~\cite{nftdefects} can detect \textit{Unlimited Minting} defect of NFTs, which share similar detection patterns. However, Pied-Piper is not fully open source (the fuzzing tool part is unavailable), and the two tools both need contract source code, while \textsc{Hyperion} only needs contract bytecode.
% In addition, our contribution lies in the detection of inconsistencies between DApp descriptions and contract implementation, the contract analysis is one of the components of our work, and our approach based on bytecode makes it more applicable as a large number of smart contracts do not reveal their source code.

\vspace{-0.2cm}
\section{Threats to Validity}
\vspace{-0.2cm}
% \subsection{Case Study}
% We give an example to show how the inconsistencies reported by \textsc{Hyperion} influence the DApp users. And how developers, users, and the DApp marketplace use our tool.

% % \vspace{-0.3cm}
% \begin{figure}[!htbp]
%     \setlength{\abovecaptionskip}{0.cm}
%     \centering
%     \includegraphics[width=\linewidth]{./images/case.jpg}
%     \caption{\textit{Fee} Inconsistency Case reported by \textsc{Hyperion}.} \label{fig:case}
% \end{figure}
% % \vspace{-0.3cm}

% Figure~\ref{fig:case} shows the DApp \textit{100k Passive} with \textit{Fee} Inconsistency reported by \textsc{Hyperion}.
% The DApp description (right of the figure) shows no information on how much fee will be charged by the contract. However, a development fee (5\%) was transferred to a preset account \verb|dev|, and the total amount of the user was subtracted by this fee without being informed. 
% The transaction~\cite{casetransaction} log on invoking the \textit{withdraw()} method on the left top of the figure shows that a user finally reaches the total amount of 344.35 BUSD but 5\% development fee (17.75 BUSD) was charged by the development fee recipient address (0x142131).
% Furthermore, the DApp also set another fee, i.e., project fee 27\% but did not mention it in the DApp description while using it in the \textit{invest()} function.
% This inconsistency can ruin the trustworthiness of DApp and hurt users' benefits as they do not perceive this subtraction of their assets.

% Our dataset includes prominent DApps like NFT projects \textit{BAYC} and \textit{CryptoKitties}~\cite{CryptoKitties}.
% In \textit{BAYC}, the contract's \textit{withdraw()} function allows the owner to withdraw all balances, but lacks clarity on emergency withdrawal conditions for user asset protection, raising trustworthiness concerns. \textit{CryptoKitties} features a pausing function controlled by top executives, impacting operations like transfers, yet this critical information is absent from its front-end description.
% More cases are shown in our repository.

% \textsc{Hyperion} serves as a practical tool for various stakeholders in the DApp ecosystem. Developers can use it to identify and rectify inconsistencies, enhancing the trustworthiness of their DApps. Users benefit by assessing a DApp's reliability, and marketplaces can leverage it to flag potentially risky DApps.

% Our dataset contains some famous DApps, e.g., NFT projects \textit{BAYC}~\cite{bayc} and \textit{CryptoKitties}~\cite{CryptoKitties}.
% Our \textsc{Hyperion} reports these two projects that contain inconsistencies.
% For the \textit{BAYC} project, we find that the contract has a function \textit{withdraw()} to control the fund flow, which allows the project owner to withdraw all the contract balance. However, there is no related information, such as in which case an emergency withdrawal will be executed to protect the user's assets, which will be considered as untrustworthiness of the DApp.
% The DApp \textit{CryptoKitties} enables the functionality of the DApp CEO/CFO/COO to pause the DApp.
% The status of the DApp will determine whether operations such as transfer can be executed normally. However, related information about DApp status is not shown in the front-end description.

% The DApp developer can utilize \textsc{Hyperion} to check whether there is inconsistency in the DApp, improving the DApp's trustworthiness.
% For normal users, they can use our tool to evaluate one DApp's trustworthiness, and the DApp marketplace can use it to identify risky DApps.

% \subsection{Limitation}
%\para{Limitations of the approach}
\para{External Validity}
% From the perspective of our approach, we find that although we utilize a higher-level representation IR, which has a complete control flow for targeted symbolic execution. As the complexity of DApps' contracts nowadays continues to rise~\cite{nftdefects}, there can be a path explosion problem, which makes it hard to reach a very deep program point.
% Furthermore, our dataflow analysis relies on Elipmoc, its ability to recover accurate dataflow information through struct data type in the future can improve our framework's performance.
Our approach, employing the symbolic execution technique, faces challenges due to the increasing complexity of DApp contracts~\cite{nftdefects}. This complexity can lead to a path explosion issue, making it difficult to analyze deeper program points. Additionally, our dataflow analysis presents a limitation in accurately recovering dataflow through struct data types.
% For the description analysis, despite our fine-tuning on the LLM, it fails to identify information in some cases. 
% This limitation is partly attributed to the inherent nature of LLMs. Their predictions or extractions can sometimes be influenced by subtleties in the data or prompt design that are not immediately apparent. Consequently, this can lead to challenges in pinpointing the exact cause of specific errors or misinterpretations by the model.
% Furthermore, in this paper, \textsc{Hyperion} only supports 7 types of inconsistency; as we design a novel and extensive framework on the contract IR, more rules can be programmed on this framework to detect more types of inconsistency in future work.
In description analysis, despite instructing-tuning the LLaMA2, we encounter instances of information misidentification. This issue partly stems from the inherent nature of LLMs, where subtle nuances in data or prompts can influence output accuracy. However, identifying specific error causes or model misinterpretations remains a challenge.
However, \textsc{Hyperion} can be improved by an instruction-tuning process with a larger labeled DApps dataset, and more rules to identify complicated data structures in the contract.

\para{Internal Validity}
% From the perspective of our experiment, the manual labeling process can also lead to mistakes, e.g., evaluation on the construction of LLM and the division of false negatives and true negatives. However, we use a double-check process to address the problem and update the labeled data set in a timely manner to ensure correctness.
% We open source all experimental results from LLM construction and evaluation on \textsc{Hyperion} with detailed markdown files.
Our manual labeling process for LLM construction and evaluation might introduce errors, particularly in differentiating between FNs and TPs. To mitigate this, we implement a double-check procedure and continuously update our dataset to ensure accuracy. All experimental results and evaluations are transparently shared in our repository.

% Despite the previous limitations, \textsc{Hyperion} still identifies many inconsistent DApps that have not been reported previously and are hard and time-consuming to identify from manual checking. Our tool \textsc{Hyperion} can help DApp developers, users, and the DApp marketplace automatically identify inconsistent DApps to improve the security of the DApp ecosystem.
% Despite these limitations, \textsc{Hyperion} effectively identifies numerous DApps inconsistencies previously unreported, which are challenging to check manually. \textsc{Hyperion} thus stands to enhance the DApp ecosystem's security, assisting developers, users, and marketplaces in identifying inconsistencies.

% (1) We only cover several kinds of fees, and from the bytecode, it is hard to map every kind of fee to the corresponding transfer operation that we find from the bycode.

% (2) We only cover 7 types of DApp inconsistencies, while there may be new types with the emerging DApps.

% \subsection{Findings}
% (1) Many of the DApps we collected in our data collection phase are not available; their websites cannot be accessed.
% It is noticeable that 100 websites of their listed DApps could not be accessible when we conducted the experiment.
% (2) Many problematic DApps, despite having varied front-end presentations, exhibit high similarities in their smart contract back-ends. And many of these DApps become unavailable when we write this paper.


==> icse2025-p517/06_related_work.tex <==
\vspace{-0.2cm}
\section{Related Work}

% There are some works that focus on unexpected behaviors in DApps.
% DAppHunter~\cite{zhou2023dapphunter} checks whether the user intention, blockchain wallet, and contract behaviors are consistent with each other. The design test logic for each DApp UI to extract user intention and focus on the transaction information of block wallet and contract. However, they do not analyze the contract bytecode or DApp descriptions.
% VetSC~\cite{duan2022towards} focuses on using DApp UI widgets to infer the DApp category and apply specific rules to implement safety vetting on contract bytecode. They just focuses some of the description while not covers the information
% {\DH}archer detects on-chain-off-chain synchronization bugs in decentralized applications~\cite{zhang2021dharcher}, which do not illustrate the DApp description and contract bytecode.
% We propose a new inconsistency scope of DApp in our paper, which exists between DApp description and contract behaviors, which are analyzed by natural language understanding and program analysis techniques, respectively.
\para{Inconsistency detection in DApps}
Several previous works focus on unexpected behaviors in DApps. For instance, DAppHunter~\cite{zhou2023dapphunter} assesses consistency among user intentions, blockchain wallet transactions, and contract behaviors, though it does not delve into contract bytecode or DApp descriptions analysis. VetSC~\cite{duan2022towards} detects discrepancies between contract bytecode and DApp category rules, deduced from the text around DApp buttons or widgets. 
% {\DH}archer~\cite{zhang2021dharcher} targets on-chain-off-chain synchronization bugs but overlooks DApp description and contract code. 
Our approach, \textsc{Hyperion}, introduces a broader scope of inconsistency, bridging the gap between DApp descriptions and contract behaviors using natural language understanding and program analysis.
% docon

\para{Smart contract security issues detection}
Recently, many program analysis tools have been developed to focus on detecting security problems in smart contracts. 
Static analysis tools like~\cite{luu2016making, mythril, rao2012sailfish} are widely used for security issue detection. Dynamic testing tools~\cite{jiang2018contractfuzzer, nguyen2020sfuzz,piedpiper}, along with machine learning approaches~\cite{zhang2022reentrancy}, also contribute to this landscape.
% \textcolor{red}{Although NFTGuard~\cite{nftdefects} and Pied-Piper~\cite{piedpiper} have similar detection patterns for the contract semantics of \textit{UTS} and \textit{UFF}, respectively, Pied-Piper is not fully open-sourced (missing fuzzing part) and NFTGuard requires the source code. In contrast, Hyperion relies solely on contract bytecode and reports issues combined with description analysis.
% We also conducted a survey on works published in top journals/conferences on SE/Security and found that the proposed inconsistencies have not been covered before (repository shows the collected list).}
However, to the best of our knowledge, \textsc{Hyperion} is the first tool incorporating both description analysis and contract semantics extraction to report newly found inconsistencies.
% Although Pied-Piper~\cite{piedpiper} can detect arbitrary transfer backdoor, and NFTGuard~\cite{nftdefects} defines a defect called Unlimited Minting, which is similar to the \textsc{Hyperion} patterns in contract analysis, 
% a complete source code of Pied-Piper~\cite{piedpiper} is not available, and all of these two tools require contract source code, while \textsc{Hyperion} can detect those issues from the bytecode.
% In addition, \textsc{Hyperion} is not only capable of contract bytecode analysis but also can analyze diverse DApp descriptions to extract user assets-related information.


\para{Inconsistency detection of traditional applications}
% Yu et al.~\cite{yu2018ppchecker} investigated the trustworthiness of privacy policies in Android apps. 
% PurPliance~\cite{datausage} was proposed to focus on the data-usage inconsistencies of an Android app, while DiffDroid~\cite{DiffDroid} was developed to find cross-platform inconsistencies in mobile apps.
% Furthermore, Ocariza et al.~\cite{ocariza2017detecting} have designed a method to identify inconsistencies in web applications.
There are some related works focusing on detecting trustworthiness and inconsistency issues in mobile~\cite{yu2018ppchecker,datausage,DiffDroid}
and web applications~\cite{ocariza2017detecting}.
However, the inexistence of a framework with rich semantics in the smart contract programming language poses unique challenges to contract bytecode analysis.

The immutable nature of blockchain transactions and financial attributes highlights the risks of DApp inconsistencies.
Our work specifically addresses this challenge and bridges the gap to enhance the DApp ecosystem's security, assisting developers, users, and marketplaces in identifying inconsistencies.

% However, in the context of DApps, the stakes of inconsistencies between front-end descriptions — often manifested as smart contract interfaces and associated documentation — and the back-end contract code's functionality are high, as the mismatch could lead to significant financial loss due to the immutable transactions on blockchain networks.
% Our work focuses on the unique environment of smart contracts and analyzing the contract bytecodes, which are open-source on the blockchain, regarding less of the code unavailability of close-source applications like Android applications.
% Furthermore, we propose a framework for detecting inconsistencies between the DApp front-end descriptions and the smart contract code, filling the gap between blockchain-based applications and providing a more secure and trustworthy ecosystem for DApp users.

==> icse2025-p517/07_conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion}
In this paper, we define seven types of DApp inconsistencies from an empirical study and introduce \textsc{Hyperion}, a tool using LLM and dataflow-guided symbolic execution to identify inconsistencies between DApp descriptions and smart contract implementations automatically. \textsc{Hyperion} instruction-tunes LLaMA2 for DApp description analysis and utilizes dataflow-guided symbolic execution for contract bytecode analysis. The experimental results show our \textsc{Hyperion}'s effectiveness in unveiling DApp inconsistencies with an overall precision of 92.06\% and an overall recall of \OverallRecall.

